Network Effects on Robustness of Dynamic Systems

We review selected results related to robustness of networked systems in finite and asymptotically large size regimes, under static and dynamical settings. In the static setting, within the framework of flow over finite networks, we discuss the effect of physical constraints on robustness to loss in link capacities. In the dynamical setting, we review several settings in which small gain type analysis provides tight robustness guarantees for linear dynamics over finite networks towards worst-case and stochastic disturbances. We also discuss network flow dynamic settings where nonlinear techniques facilitate in understanding the effect on robustness of constraints on capacity and information, substituting information with control action, and cascading failure. We also contrast the latter with a representative contagion model. For asymptotically large networks, we discuss the role of network properties in connecting microscopic shocks to emergent macroscopic fluctuations under linear dynamics as well as for economic networks at equilibrium. Through the review of these results, the paper aims to achieve two objectives. First, to highlight selected settings in which the role of interconnectivity structure of a network on its robustness is well-understood. Second, to highlight a few additional settings in which existing system theoretic tools give tight robustness guarantees, and which are also appropriate avenues for future network-theoretic investigations.

==> capacity-dynamic/network-flow-dynamics.tex <==
\section{Robustness of Network Flow to Perturbation in Capacity: Dynamical Setting}
\label{sec:capacity-perturbation-dynamic}
Recall the notions of super source and super sink from Section~\ref{sec:notations}. It is convenient to identify them both with the same virtual node, say $0$. Add a virtual directed link $(0,v)$ from the virtual node to every source node $v \in \mc V$; let this set be denoted as $\linkin$. Similarly add a virtual directed link $(v,0)$ from every sink node $v \in \mc V$ to the virtual node; let this set be denoted as $\linkout$.
%Let the augmented set of nodes and directed links be denoted as $\tilde{\mc V}$ and $\tilde{\mc E}$ respectively. 
We consider the following class of network flow dynamics corresponding to mass conservation:
\begin{equation}
\label{eq:network-flow-dynamics-general}
\dot{x}_i = \underbrace{\sum_{j \in \mc E \cup \linkin} \interflow_{ji}(x)}_{\text{inflow}} - \underbrace{\sum_{j \in \mc E \cup \linkout} \interflow_{ij}(x)}_{\text{outflow}}, \qquad i \in \mc E
\end{equation}
%
% \begin{equation}
% \label{eq:network-flow-dynamics-general}
% \dot{x} = \underbrace{\lambda + R^T(x)f(x,c)}_{\text{inflow}} - \underbrace{f(x,c)}_{\text{outflow}}
% \end{equation}
 where $x_i \geq 0$ denotes the mass on link $i \in \mc E$, and $\interflow_{ij} \geq 0$ is the flow from link $i \in \mc E \cup \linkin$ to link $j \in \mc E \cup \linkout$. Naturally, $\interflow_{ij}=0$ if $i$ is not incident to $j$. The $\interflow_{ij}$'s depend on the state $x$, and this dependence is typically induced by a state feedback control; the exact model depends on the setting.  Sections~\ref{sec:routing}, \ref{sec:routing+scheduling} and \ref{sec:scheduling} consider a few such canonical settings. In all these settings, $\interflow_{ij}$'s are constrained to be such that $\interflow_{ij}(x)=0$ for all $j$ if $x_i=0$,  and $\sum_{j \in \mc E \cup \linkout} \interflow_{ij}(x) \leq c_i$ if $i \in \mc E$ and $\sum_{j \in \mc E \cup \linkout} \interflow_{ij}(x) = \lambda_i$ if $i \in \linkin$. The first constraint ensures that \eqref{eq:network-flow-dynamics-general} is a positive system, i.e., $x(t) \geq \zerobf$ for all $t$, the second constraint implies that the total outflow from an actual link is upper bounded by its capacity (analogous to the static network flow setting described in Section~\ref{sec:notations}), and third constraint specifies the total external flow coming into source nodes. 
 %These constraints will be collectively denoted as $\interflowconstraints$. 
 %Let these constraints be succinctly denoted as $\{f_{ij}\}_{ij} \in \mc F$.  
% $f(.) \in \reals_{\geq 0}^{\mc E}$ denotes link outflows, and $\lambda \in \reals_{\geq 0}^{\mc E}$ denotes external inflows to the links. $R(.)$ is a row sub-stochastic matrix denoting the routing of flow among the links, i.e., $R_{ij} \in [0,1]$ denotes the fraction of outflow from $i \in \mc E$ which contributes to inflow of $j$, and $\sum_{j \in \mc E} R_{ij} \leq 1$ for all $i \in \mc E$, with $1-\sum_{j \in \mc E}R_{ij}$ being the fraction of the outflow from $i$ leaving the network. These features of $R$ ensure flow conservation at every node in the network. $R(.)$ and $f(.)$ are controlled quantities, where $R(.)$ is constrained to satisfy the aforementioned row sub-stochastic property, and one can constrain $f(.)$ to satisfy $f_i(.)=0$ if $x_i=0$, for all $i \in \mc E$, to impose positivity on \eqref{eq:network-flow-dynamics-general}, i.e., $x(t) \geq \zerobf$ for all $t$. Additionally, $f(.)$ is constrained to satisfy $f(.) \leq c$, where the parameters $c \in \reals_{>0}^{\mc E}$ denote link-wise capacities. Let such constraints be succinctly denoted as $R(.) \in \mc R$ and $f(.) \in \mc F$. 
It is of interest to study stability of \eqref{eq:network-flow-dynamics-general} and robustness to perturbations in $\{c_i\}_{i \in \mc E}$ under different models for $\{\interflow_{ij}(x)\} \in \interflowconstraints$. 
 
 
\subsection{Routing Control for Single Commodity Flow}
\label{sec:routing} 
It is natural to consider the decomposition $\interflow_{ij}(x)=f_i(x) R_{ij}(x)$, where $f_i(x) \geq 0$ is the net outflow from $i \in \mc E \cup \linkin$ satisfying $f_i(x)=0$ if $x_i=0$ for all $i$, $f_i(x) \leq c_i$ for all $i \in \mc E$ and $f_i(x) \equiv \lambda_i$ for all $i \in \linkin$, and $R_{ij}(x) \in [0,1]$ is the routing function satisfying $R_{ij}(x) \equiv 0$ if $i$ is not incident to $j$, and $\sum_{j} R_{ij}(x) \equiv 1$ for all $i$. 
One can simplify the model further by letting $f_i(x) \equiv f_i(x_i)$ be strictly increasing for all $i \in \mc E$, and $R_{ji}(x)\equiv R_{ki}(x)\equiv R_i(x)$ for any two links $j$ and $k$ incident on to $i$. The first assumption implies that the outflow from $i$ depends only on mass on $i$ and is increasing with respect to it, and the latter assumption implies that each node adds flow from immediate upstream links and instantaneously routes it among its immediate downstream links, without consideration for the source or destination of that flow. This naturally makes sense for a \emph{single commodity} flow. For simplicity in presentation, we assume single source and single sink. Extension to multiple sources and sinks, for single commodity flow, follows from the construction in Section~\ref{sec:notations}. Correspondingly, we shall remove subscript and let $\lambda$ denote the external flow to the only source node. We make the following assumption in this section and the next:
\begin{assumption}
\label{ass:connectivity-general}
For every node $v \in \mc V$, there exists a directed path from the source node to $v$ and from $v$ to the sink node.
\end{assumption}

In the current setting, the stability and robustness properties of the network flow dynamics depend on the choice of routing functions $R$. Of particular interest is decentralized routing where the routing control action for a link depends only on the state on $i$ and on links having the same tail node as $i$, i.e., $R_i(x) \equiv R_i(\{x_j: \, j \text{ and } i \text{ have same tail node}\})$. Consider a feasible flow $f^*$, i.e., satisfying the flow conservation and capacity constraints, and correspondingly $\{x_i^*:=f_i^{-1}(f_i^*)\}_{i \in \mc E}$. Given such $x^*$ and $f^*$, which exist if and only if $\lambda$ is less than the minimum cut capacity of the network, consider decentralized routing control satisfying: (i) $R_i(x^*)=\frac{f_i^*}{\sum_{j}f_j^*}$ for all $i \in \mc E$, where the summation is over all links $j$ which have the same tail node as $i$, and (ii) $\frac{\partial R_i(x)}{\partial x_j} >0$ for every two distinct links $i$ and $j$ having the same tail node. (i) implies that $x^*$ is an equilibrium. (ii) implies that, if $x_j$ increases but the state on other links which affect $R_i$ remain the same, then more flow will be routed to every other link. This property helps to establish global asymptotic stability of $x^*$ if $\mc G$ is acyclic. This is because (ii) along with increasing nature of $f_i(.)$ implies that the Jacobian of \eqref{eq:network-flow-dynamics-general} under these conditions is a compartmental matrix, i.e., a Metzler matrix whose column sums are non-positive. Such systems are known to possess a contraction principle, e.g., see \cite{Sontag:10}. 

The (decentralized) routing satisfying (i) and, particularly, (ii) above is referred to as \emph{monotone}  routing. An example of monotone routing is:
\begin{equation*}
R_i(x) = \frac{f_i^* e^{\beta(x^*_i-x_i)}}{\sum_j f_j^* \exp(\beta(x^*_j-x_j))}, \quad \beta>0
\end{equation*}
which is the multinomial logit model at node $v$ for choosing among links in $\mc E_v^+$, when the utility function associated with $i \in \mc E_v^+$ is $x_i^*-x_i+\log f_i^*$. Indeed, monotone routing is interpreted as en route driver decision in \cite{Como.Savla.ea:SICON11}, with $x^*$ being the nominal network state expected by the drivers during the trip. This nominal state is updated by the driver population at a slower time scale according to a best response rule, e.g., see \cite{Sandholm:10}. The link (out-)flows under such a multi-scale update rule are shown to converge to a Wardrop equilibrium in \cite{Como.Savla.ea:SICON11}, if $\mc G$ is acyclic, and if each $f_i(.)$, $i \in \mc E$, is strictly concave in addition to being strictly increasing. 

The monotone routing policies are also shown to admit the following sharp characterization of robustness of equilibrium $x^*$ to perturbation in capacity~\cite{Como.Savla.ea:Part1TAC10,Como.Savla.ea:Part2TAC10}. Let $\triangle \in [0,c]$ denote the perturbation in capacity. Clearly, there exists a $\|\triangle\|_1$ (infinitesimally) greater than the network residual capacity, such that at least one component of $x(t)$ grows unbounded for every (not necessarily decentralized) routing policy. Such a $\triangle$, e.g., corresponds to reducing capacities on the links outgoing from the minimum cut by infinitesimally greater than the residual capacities on them. However, if the routing policy is decentralized, such as the monotone routing, then reducing capacities on the links, outgoing from the node having the smallest residual capacity, by an amount infinitesimally greater than their respective residual capacities is sufficient to ensure that $x_i(t)$ grows unbounded at least for one $i \in \mc E$. 
Interestingly, under the monotone routing, if $\mc G$ is acyclic, then for \emph{every} $\|\triangle\|_1$ less than the minimum node residual capacity, there exists a globally asymptotically stable equilibrium, which is different than the equilibrium $x^*$ associated with the nominal, i.e., non-perturbed system. The existence of a new equilibrium is established by a novel use of the monotonicity property of the underlying dynamics (cf. \cite{Como.Savla.ea:Part2TAC10}), and the stability then follows from the contraction principle, along the same lines as the stability of nominal dynamics. 

\subsection{Routing and Scheduling Control for Single Commodity Flow} 
\label{sec:routing+scheduling}
Consider again the single commodity flow setting with a single source single and a single sink (without loss of generality) from Section~\ref{sec:routing} as well as Assumption~\ref{ass:connectivity-general}. 
Recall that, in Section~\ref{sec:routing}, the outflow from a link was uncontrolled and determined by $\{f_i(x_i)\}_{i \in \mc E}$. Let us relax this feature, but maintain the decentralization aspect. 
That is, we let $\interflow_{ij}(x)$ be controlled, and let $\interflow_{ij}(x) \equiv \interflow_{ij}(\{x_k: \, k \text{ has the same head node as } i \text{ or the same tail node as }j\})$. An implication of the relaxation is that  we extend the scope of control to also determine the outflow from a link in addition to determining the routing part. A natural extension of the monotonicity property from Section~\ref{sec:routing} to the current setting is to consider decentralized $\{\interflow_{ij}\}$ which satisfy the following for all $i \in \mc E \cup \linkin$ and $j \in \mc E \cup \linkout$: (i)  $\frac{\partial \interflow_{ij}(x)}{\partial x_k} >0$ for all $k$, except $j$, which has the same head node as $i$ or the same tail node as $j$, and (ii) $\frac{\partial \sum_{j} \interflow_{ij}(x)}{\partial x_k} <0$ for all $k$ to which $i$ is incident. These properties imply that if $x_k$ increases, but the state on the other links which affect $\interflow_{ik}$ remains the same, then (i) more flow is sent to links other than $k$, but which have the same tail node as $k$, and (ii) the total outflow $\sum_{j} \interflow_{ij}(x)$ from every link $i$ incident on to $k$ decreases. We call the control policies $\{\interflow_{ij}(x)\}$ satisfying these two properties as \emph{monotone control policies} (in contrast to monotone \emph{routing} policies in Section~\ref{sec:routing}) with a slight abuse of terminology. An example of monotone control is:
$$
\interflow_{ij}(x) = c_i \left(1 - e^{- \beta x_i} \right) \frac{e^{- \beta x_j}}{\sum_k e^{-\beta x_k}}, \qquad \beta>0
$$
where the summation is over all $k$ which have the same head node as $i$ or the same tail node as $j$. 

In \cite{Como.Lovisari.ea:TCNS13}, using similar tools as described in Section~\eqref{sec:routing}, it is shown that, under monotone control, if $\lambda$ is less than the min cut capacity, then there exists a globally asymptotically stable equilibrium $x^*$. An implication of this is that, for all perturbations to capacity $\|\triangle\|_1$ less than the network residual capacity, there exists a globally asymptotically stable (new) equilibrium under monotone control. Combining this with the fact that, there exists $\triangle$ with $\|\triangle\|_1$ (infinitesimally) greater than the network residual capacity such that no controller (not necessarily decentralized) can prevent $x(t)$ from growing unbounded on at least one component implies that monotone control policies are maximally robust to perturbation in capacity among all (not necessarily decentralized) controllers. This robustness guarantee is stronger than the one on monotone routing policy in Section~\ref{sec:routing} which further required acyclic assumption on $\mc G$. 
Moreover, the monotone routing is parameterized by equilibrium $x^*$ and hence requires some kind of centralized coordination, whereas no such coordination is required in the current monotone control setting. The additional control action in the current setting in the form of scheduling, in conjunction with property (ii) in the definition of monotone control, allows for forward \emph{and} backward propagation of dynamics. Interestingly, such propagations are sufficient to compensate for the decentralization feature of the controller to give as good robustness performance as any centralized controller. On the other hand, the lack of scheduling action in the setting of Section~\ref{sec:routing} allows only forward propagation of dynamics resulting in gap in robustness guarantees with respect to a centralized controller. 

\cite{Como.Lovisari.ea:TCNS13} also considers a few extensions, most notable being consideration of finite storage capacity on the links, i.e., $x(t) \leq B \in \reals_{>0}^{\mc E}$. 
If $\lambda$ is less than the minimum cut capacity (which is a necessary condition for boundedness of $x(t)$), it is shown that there exists a globally asymptotic stable equilibrium  under appropriate modification of the monotone controller. It is also shown that, under such a modified controller, if the necessary condition does not hold true, then there exists a cut such that all links outgoing from that cut hit their respective storage capacities (which are not necessarily equal) simultaneously. This possibly suggests \emph{graceful degradation} in the unstable regime, i.e., maximizing the time till any link hits storage capacity which could cause link failure. 
 
\cite{Coogan.Arcak:Automatica15} presents an another setting where the concept of monotonicity is useful for tight stability analysis. However, not all practical variants of \eqref{eq:network-flow-dynamics-general} are amenable to such analysis. The next section discusses such an important class of network flow dynamics.
 
\subsection{Scheduling Control for Multiple Commodity Flow}
\label{sec:scheduling}
Recall that, in Sections~\ref{sec:routing} and \ref{sec:routing+scheduling}, we considered single commodity flow. 
%
%\kscomment{(single source and)} single sink setting, which can be trivially extended to multi source multi sink setting for single commodity flow, as noted in Section~\ref{sec:notations}. However, 
Multiple commodity setting imposes constraint on the flow that needs to be routed between every source-sink pair. One way to model this is by fixing the routing matrix. Accordingly, we revisit the decoupling of $\interflow_{ij}$ from Section~\ref{sec:routing} as $\interflow_{ij}(x)=f_i(x) R_{ij}$, and consider multiple sources and multiple sinks. We remove $\linkin$ and let the external flow arrive directly on to the links outgoing from the source nodes. In summary, in the current setting, \eqref{eq:network-flow-dynamics-general} becomes:
\begin{equation}
\label{eq:network-flow-dynamics-scheduling}
\dot{x} = \lambda + \left(R^T - I \right) f(x) 
\end{equation}
where $\lambda \in \reals_{\geq 0}^{\mc E}$ is the external inflows at the links, and, with a slight abuse of notation, $R$ denotes the routing sub-matrix restricted to links in $\mc E$. The following is the natural extension of Assumption~\ref{ass:connectivity-general}.
\begin{assumption}
\label{ass:connectivity-scheduling}
For every node $v \in \mc V$, there exists a directed path from at least one source node to $v$, and there exists a directed path from $v$ to at least one sink node.
\end{assumption} 
Motivated by scenarios involving allocation of a fixed service resource to multiple conflicting queues, e.g., at a signalized traffic intersection in urban traffic networks or at a router in communication networks, consider the following simple model for link outflows:
\begin{equation}
\label{eq:outflow-scheduling}
f_i(x) \equiv f_i(x_i)= \Big \{\begin{array}{ll}
u_i(x) c_i & \text{ if }x_i > 0 \\
\sum_{j} R_{ji} f_j(x) & \text{ if }x_i=0
\end{array}, \qquad i \in \mc E
\end{equation}
where the summation is over all links $j \in \mc E \cup \linkin$ that are incident to $i$. The control input $u_i(x) \in [0,1]$ can be interpreted as the fraction of times that the queue on $i$ gets serviced. \eqref{eq:outflow-scheduling} ensures positivity of \eqref{eq:network-flow-dynamics-scheduling} in the current setting. The fixed resource feature is modeled by imposing 
\begin{equation}
\label{eq:finite-resource}
\sum_{i \in \mc E_v^-} u_i(x) \leq 1,  \quad  v \in \mc V
\end{equation}
%where, in this setting, $\mc E_v^-$ also includes links in $\linkin$ whose head node is $v$. 
By further imposing $u_i(x) \to 0^+$ as $x_i \to 0^+$ (and starting from an initial condition $x_0 > \zerobf$), one can ensure that the $x_i=0$ case in \eqref{eq:outflow-scheduling} is never active, and thereby also avoiding regularity issues with the right hand side of \eqref{eq:network-flow-dynamics-scheduling}.

A necessary condition for the boundedness of $x(t)$, and hence also for the existence of equilibrium, in the current setting, is $\sum_{i \in \mc E_v^-} \frac{f_i^*}{c_i} \leq 1$ for all $v \in \mc V$, where $f^*$ is the flow \emph{induced} by $\lambda$ and $R$, i.e., $\lambda+(R^T-I)f^*=0$, which implies $f^*=(I-R^T)^{-1} \lambda$, where invertibility is guaranteed by Assumption~\ref{ass:connectivity-scheduling}. It is of interest to study stability conditions under natural controllers $u(x)$ and compare with the necessary condition. It is straightforward to see that, if the necessary condition is satisfied, then the open-loop controller $u_i(x) \equiv f_i^*/c_i$, $i \in \mc E$, satisfies \eqref{eq:finite-resource}, and, under it,  every $x>\zerobf$ is an equilibrium of \eqref{eq:network-flow-dynamics-scheduling}. Besides being an open-loop, this controller requires information about $\lambda$ and $R$ and is therefore centralized. In parallel to Sections~\ref{sec:routing} and \ref{sec:routing+scheduling}, it is of interest to study decentralized controllers of the form: $u_i(x) \equiv u_i(x_j: \, j \text{ has the same head node as }i)$. Using monotonicity arguments similar to Sections~\ref{sec:routing} and \ref{sec:routing+scheduling}, it is shown in \cite{Savla.Lovisari.ea.Allerton13} that, if $\mc G$ is acyclic and if the necessary condition is satisfied, then, under the following controller, there exists a unique $x^* > \zerobf$ whose basin of attraction is $\reals_{>0}^{\mc E}$:  
\begin{equation}
\label{eq:pf-controller}
u_i(x) = \frac{x_i}{\sum_{j} x_j + \beta}, \qquad \beta>0
\end{equation}
where the summation is over all $j$ with the same head node as $i$. Extension of this result to cyclic $\mc G$ is provided in \cite{Nilsson.Hosseini.ea.CDC15} by establishing $\sum_{i \in \mc E} x_i \log \left( u_i(x) \frac{c_i}{f_i^*}\right)$ as Lyapunov function. Indeed, the inspiration for this analysis comes from the literature on stochastic networks, e.g., see \cite{Massoulie:07}, where \eqref{eq:pf-controller} is interpreted as a \emph{proportionally fair} controller for the current setting. It is remarkable to note that the decentralized controller in \eqref{eq:pf-controller} gives the same stability guarantee as the centralized (open-loop) controller without requiring information about (even local) $\lambda$, $R$ or $c$. The literature on back pressure controllers, e.g., see \cite{Tassiulas.Ephremides:92}, suggests that one can get the same stability guarantee by establishing $\sum_{i \in \mc E} x_i^2$ as Lyapunov function. 
 Such tight stability guarantees translate into tight guarantees on robustness to perturbation to link capacities, along the lines of Section~\ref{sec:routing+scheduling}. 



==> capacity-static/dc-networks.tex <==
\ksmarginsoft{replace some text with theorem in Sections~\ref{sec:capacity-perturbation-static} and \ref{sec:capacity-perturbation-dynamic}}
\section{Robustness of Network Flow to Perturbation in Capacity: Static Setting}
\label{sec:capacity-perturbation-static} 
We now consider robustness of network flow to perturbation in link capacities. Since the quantity of interest, i.e., flow, is associated with links, for brevity in notation, we switch the indices used for nodes in previous sections to links. Accordingly, link flows, weights, and capacities will, respectively, be denoted as $f=\{f_i\}_{i \in \mc E}$, $\mc W=\{\mc W_i\}_{i \in \mc E}$ and $c=\{c_i\}_{i \in \mc E}$. 
The starting point for robustness analysis is the max flow min cut theorem for the standard static formulation, as described in Section~\ref{sec:notations}. Formally, consider the \emph{nominal} scenario where an inflow of $\lambda>0$ is routed from $s$ to $t$. $\lambda$ is less than the solution to the maximum flow problem, and hence there exists a feasible flow whose value is equal to $\lambda$. Let the link capacities be reduced by $\triangle \in [0,c]$. If $\|\triangle\|_1$ is less than the residual capacity of the unperturbed network, then there exists a new flow that is feasible for the perturbed network, i.e., it is less than $c-\triangle$ and satisfies \eqref{eq:flow-conservation}, with the same value $\lambda$. On the other hand, there exists a $\|\triangle\|_1$ infinitesimally greater than the network residual capacity, corresponding to reducing capacity on links outgoing from the minimum cut infinitesimally greater than their respective residual capacities, under which such a feasible flow is not possible for the perturbed network. It is of interest to extend such robustness analysis to additional constraints on flow and in presence of control.

The first extension that we consider is motivated by electrical networks. In order to model bi-directionality of electrical flow, while continuing to adopt the directed graph formulation of network flow from Section~\ref{sec:notations}, we do not constrain the entries of flow $f$ to be non-negative. 
%The capacity constraints can then be rewritten as $|f_i| \leq c_i$ for all $i \in \mc E$. 
In addition to \eqref{eq:flow-conservation} (Kirchhoff current law), the flow is constrained to also satisfy Ohm's law. Formally, $f \in \reals^{\mc E}$ is said to satisfy the physical constraints if there exist (voltage angles) $\phi \in \reals^{\mc V}$ such that $f=\incidence \biglambda$ and $f=\diag(\mc W) \incidence^T \phi$, where $\biglambda \in \reals^{\mc V}$ is such that $\Lambda_v$ is equal to $\lambda$ (resp., $-\lambda$) if $v$ is the source (resp., sink), and is equal to zero otherwise. This corresponds to interpreting $f$ as DC approximation to power flow, with $\mc W$ being the negative of link susceptances.  
If $\mc G$ is weakly connected, then such a unique $f$ always exists, and is given by 
\begin{equation}
\label{eq:electrical-flow}
f(\mc W,\Lambda)=\diag(\mc W) \incidence^T L^{\dagger} \Lambda
\end{equation}
 where $L^{\dagger}$ is the Moore-Penrose pseudo-inverse of the weighted Laplacian $L:=\incidence \diag(\mc W) \incidence^T$. Noting the linear dependence of $f(\mc W,\Lambda)$ on $\Lambda$, and hence $\lambda$, it is easy to see that, given $c$ and $\mc W$, the maximum flow problem in this setting can again be cast as a linear program. Let the solution be denoted as $\lambdamax(\mc W)$. A generalization of this is when the link weights are flexible: $\mc W \in [\Wmin, \Wmax]$, with $\Wmax \geq \Wmin \geq \zerobf$. It is then of interest to study $\max_{\mc W \in [\Wmin,\Wmax]} \lambdamax(\mc W)$, and the corresponding maximizing $\mc W$. The solution to this problem can be naturally interpreted in terms of robustness to perturbation to capacity under \emph{controllable} link weights, in the same spirit as the max flow min cut theorem described earlier in this section.  

The technical challenge is due to the nonlinear dependence of $f$, and hence also of $\lambdamax$, on $\mc W$. 
\cite{Ba.Savla:TCNS16} presents an incremental network reduction approach to reduce the complexity of this problem. In the classical network flow framework (cf. Section~\ref{sec:notations}), replacing the network with a directed link from $s$ to $t$ whose capacity is the solution to the maximum flow problem is equivalent from capacity perspective. The notion of Thevenin equivalent resistance allows to replace the electrical network having link-wise weights $\mc W$ with an equivalent link with weight $\Weq$. The equivalence then maps $[\Wmin,\Wmax] \subset \reals_{\geq 0}^{\mc E}$ to, say, $[\Wmin^{\mathrm{eq}},\Wmax^{\mathrm{eq}}] \subset \reals_{\geq 0}$, and it can be shown that $\Wmin$ (resp., $\Wmax$) maps to $\Wmin^{\mathrm{eq}}$ (resp., $\Wmax^{\mathrm{eq}}$). The following rewriting:
\begin{equation}
\label{eq:max-capacity}
\max_{\mc W \in [\Wmin,\Wmax]} \lambdamax(\mc W) = \max_{\Weq \in [\Wmin^{\mathrm{eq}},\Wmax^{\mathrm{eq}}]} \lambdamax(\Weq)
\end{equation}
with $\lambdamax(\Weq):=\max\{\lambdamax(\mc W): \, \mc W \in [\Wmin, \Wmax] \text{ s.t. equivalent weight of $\mc W$ is } \Weq\}$ suggests $\lambdamax(\Weq)$ as the capacity associated with $\Weq$. This notion of capacity lends itself to the following iterative solution of \eqref{eq:max-capacity} if $\mc G$ is \emph{tree reducible}, i.e., if $\mc G$ can be reduced to a single link by a sequence of series and parallel subnetwork reductions, as illustrated in Figure~\ref{fig:network-reduction}(a). \cite{Ba.Savla:TCNS16} shows that a particular quasi-concave property of capacity functions $\lambdamax(.)$ remains invariant across each of these reduction steps, see Figure~\ref{fig:network-reduction}(b).  Moreover, the interval over which the capacity function for a network achieves its maximum can be analytically related to the corresponding intervals of its sub-networks, thereby allowing an analytical solution to \eqref{eq:max-capacity}, which is a non-convex problem, for tree reducible $\mc G$. For other $\mc G$, one can perform this reduction for each of tree-reducible sub-networks of $\mc G$ to equivalently reducing the size of \eqref{eq:max-capacity}, and thereby reducing computational complexity. 
\begin{figure}[htb!]
\begin{minipage}[c]{.67\textwidth}
\begin{minipage}[c]{.22\textwidth}
\begin{center}
\includestandalone[width=0.9\linewidth]{./fig/tree-reducible-net}
\end{center}
\end{minipage} $\to$
\begin{minipage}[c]{.215\textwidth}
\begin{center}
\includestandalone[width=0.9\linewidth]{./fig/tree-reduced-1}
\end{center}
\end{minipage} $\to$
\begin{minipage}[c]{.195\textwidth}
\begin{center}
\includestandalone[width=0.9\linewidth]{./fig/tree-reduced-2}
\end{center}
\end{minipage} $\to$
\begin{minipage}[c]{.185\textwidth}
\begin{center}
\includestandalone[width=0.9\linewidth]{./fig/tree-reduced-3}
\end{center}
\end{minipage}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center} \hspace{-0.3in}
\includestandalone[width=0.75\linewidth]{./fig/capacity-function-reduction-overlay}
\end{center}
\end{minipage}
\begin{minipage}[c]{.67\textwidth}
\begin{center}
(a)
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
(b)
\end{center}
\end{minipage}
\caption{(a): sequence of network reductions for a tree reducible graph (b): corresponding capacity functions}
\label{fig:network-reduction}
\end{figure}





==> cascading-failure/cascading-failure-main.tex <==
\section{Cascading Failure}

\input{./cascading-failure/cascading-failure-network-flow}

\input{./cascading-failure/cascading-failure-contagion}

It is interesting to note a couple of differences between the formulations in Sections~\ref{sec:cascading-failure-network-flow} and \ref{sec:cascading-failure-contagion}. First, the cascade process in Section~ \ref{sec:cascading-failure-contagion} propagates from a node to its neighbors from one instant to the next. This localized feature is to be contrasted from Section~\ref{sec:cascading-failure-network-flow}, where, following the failure of link(s), the next link(s) to fail as a result (as determined by the physical laws and control) are not necessarily adjacent to the link(s) that failed in the previous instant. Second, the threshold assignment in Section~\ref{sec:cascading-failure-contagion} is independent of the graph structure or the process which led to it. This is to be contrasted with Section~\ref{sec:cascading-failure-network-flow}, where the vulnerability of a link is related to its residual capacity with respect to the nominal equilibrium flow, and hence is dependent on the process which yields the equilibrium flow. 

==> non-asymptotic-dynamic/flow/analysis.tex <==
\subsection{Analysis}
The results in this section are inspired by \cite{Wang.Elia:12}.

\begin{theorem}
\label{thm:stable-main}
\eqref{eq:structured-uncertainty-form} is MS stable, if and only if either of the following conditions hold:
\begin{enumerate}
\item[(a)] $\exists \, X > 0$ such that $\mc H (X)< X$, where 
\begin{equation}
\label{eq:H-def}
\mc H(X):=\Amatrix X \Amatrix^T + \sum_{j=1}^m \sigma^2_{\gamma_j} A^{(j)} X {A^{(j)}}^T
\end{equation}
\item[(b)] $\rho(\mc H)<1$
%\begin{equation}
%\label{eq:spectral-radius-condition}
%\rho(\mc H)<1
%\end{equation}
%
%$\rho(\mc H)<1$, where
%$$
%\mc H:=AXA^T + \sum_i \sigma_i^2 B(i) C_i X C_i^T B^T(i)
%$$
%\item[(c)] The mean system $G$ is stable (cf Definition~\eqref{eq:mean-system}) and satisfies $\rho(\|G\|_2^2 \Sigma)<1$
%where 
%$$
%\|G\|_2^2 = \begin{bmatrix}
%\|G_{11}\|_2^2 & \ldots & \|G_{1m}\|_2^2 \\
%\vdots & \ldots & \vdots \\
%\|G_{m1}\|_2^2 & \ldots & \|G_{mm}\|_2^2
%\end{bmatrix}
%$$
%and $\Sigma$ is the covariance matrix of $\bigtriangle$.
\end{enumerate}
\end{theorem}

\ksmargin{can we get rid of $\sigma_w=0$?}
\kscomment{
If $\sigma_w=0$}, then MS stability implies that $x(t) \to 0 $ almost surely, and $E[x(t)] \to 0$. The converse is established as follows.

%\begin{definition}
%\eqref{eq:structured-uncertainty-form} is said to be MS \kscomment{convergent} if, under $w(t) \equiv 0$, $E x(t) \to 0$. 
%\end{definition}

\begin{proposition}
\label{prop:stable}
Consider \eqref{eq:structured-uncertainty-form} with $\sigma_w=0$. $E[x(t)] \to 0$ if and only if \eqref{eq:structured-uncertainty-form} is MS stable. 
\end{proposition}

The next result gives further insight into the behavior when \eqref{eq:structured-uncertainty-form} is MS unstable.



\begin{theorem}
\label{thm:unstable}
Let Assumption~\ref{ass:connectivity} hold true. If \eqref{eq:structured-uncertainty-form} is MS unstable, then $\lim_{t \to \infty} E[(x_i(t)-x_i(t-1))^2] = \infty$ for all $i \in \mc V$.
%The following results hold true.
%\begin{enumerate} 
%\item[(a)] 
%$\lim_{t \to \infty} E[x_i(t)] = \infty$ and 
%\item[(b)] Let \kscomment{$\eta < 0$}. \kscomment{$x_i(t)$ (or $x_i(t)-x_i(t-1)$?)} converges in distribution to a random variable $R_i$, for all $i \in \mc V$, as $t \to \infty$. Furthermore, $R_i$ has unbounded second moment if and only if \eqref{eq:structured-uncertainty-form} is MS unstable.
%\end{enumerate}
\end{theorem}



==> non-asymptotic-dynamic/flow/computations.tex <==
\subsection{Computations}
The following procedure is adapted from \cite{Bamieh.Filo:18}. To calculate the spectral radius of $\mc H$ defined in \eqref{eq:H-def}, one can find the largest real number $\lambda$ which satisfies the following 
\begin{equation*}
\label{eq:LMI}
\begin{split}
\lambda \left(X - \Amatrix X \Amatrix^T \right) - \sum_{j=1}^m \sigma^2_{\gamma_j} A^{(j)} X {A^{(j)}}^T & = 0 
\\
X & \geq 0
\end{split}
\end{equation*}

==> non-asymptotic-dynamic/flow/conclusion.tex <==
\subsection{Extensions}
\begin{enumerate}
\item non-diagonal $\bigtriangle$
\item non-linear network flow dynamics in \cite{Como.Savla.ea:Part1TAC10} and \cite{Como.Lovisari.ea:TCNS13}
\item vector $w(t)$
\item $w(t)$ as non-negative r.v.
\item enforce non-negativity on $x(t)$
\end{enumerate}

==> non-asymptotic-dynamic/flow/notations.tex <==
\subsection{Notations}
$I_n$ is the identity matrix of size $n$. For a matrix $A$, $A_i$ denotes its $i$-th row, and $A(i)$ denotes its $i$-th column. $\mc V$ denotes the set of nodes. $[m]$ is short hand for $\{1, \ldots, m\}$.

==> non-asymptotic-dynamic/flow/simulations.tex <==
\subsection{Simulations}
Consider the setup of Example~\ref{example:linear-transportation-network}, with the $(1,1)$ entry of $A^{(0)}$ set to $-\ell_{31}$. The parameters are chosen as: $\ell_{31}=1$, $\ell_{12}=0.1$, $\ell_{32}=0$, $\ell_{23}=0.1$, $\ell_{43}=3$, $\ell_{34}=1$, $\mu_{\gamma_1}=0.1$. Figure~\ref{fig:sim} (left) is for $B_w=\zerobf$ (i.e., noiseless case), and Figure~\ref{fig:sim} (right) is for $B_{w}=0.1 \onebf$ (i.e., small additive noise). 

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.475\textwidth]{./fig/noiseless}
\includegraphics[width=0.475\textwidth]{./fig/withnoise}
\end{center}
\caption{\sf Simulation Results.}
\label{fig:sim}
\end{figure}

==> non-asymptotic-dynamic/flow/stochastic-uncertainty-problem-formulation.tex <==
\subsection{Problem Formulation}
Consider the following linear network flow dynamics:
\begin{equation}
\label{eq:routing-discrete-time}
x(t+1) = x(t) + \tilde{A}(t)x(t) + B_w w(t)
\end{equation}
where $x \in \real_{\geq 0}^n$ is the state of the system, the routing matrix $\tilde{A}(t)$ is a matrix-valued random process, independent of $\{x(\tau), \, \tau \leq t\}$; and $w(t)$ is a scalar (for simplicity) random process, independent of $\tilde{A}(t)$. We shall consider a particular form of \eqref{eq:routing-discrete-time} using scalar-valued random processes $\gamma_1, \ldots, \gamma_m$ as follows:
\begin{align}
x(t+1) & = \left(I + A^{(0)} + A^{(1)} \gamma_1(t) + \ldots + A^{(m)} \gamma_m(t) \right) x(t) + B_w w(t) \nonumber \\
\label{eq:routing-discrete-time-reformulation}
& = \left(I + A^{(0)} + \sum_{j=1}^m \mu_{\gamma_j} A^{(j)} \right) x(t) + \left(\sum_{j=1}^m \triangle_j(t) A^{(j)} \right) x(t) + B_w w(t)
\end{align}
%where $m$ is the number of links associated with uncertainty, $\gamma_j(t):=\mu_{\gamma_j} + \triangle_j(t)$ for all $j \in [m]$, with $\mu_{\gamma_j}$ being the mean of $\gamma_j(t)$, and \kscomment{$A_0, A_1, \ldots, A_m$ are Metzler matrices.} \ksmargin{is Metzler stuff true?} \kscomment{For simplicity, we let $\gamma_j$ be Bernoulli random variables.} \ksmargin{where is this used?}

$A^{(0)}, A^{(1)}, \ldots, A^{(m)}$ can be given the following interpretation. $A^{(0)}$ corresponds to the dynamics with no uncertainty, whereas each of $A^{(j)}$, $j \in [m]$ corresponds to an uncertain link, or possibly different levels of uncertainty of the same link; see Example~\ref{example:linear-transportation-network}. Each of $A^{(0)}, A^{(1)}, \ldots, A^{(m)}$ is a Metzler matrix, and induces a sub-graph over the complete directed graph over the node set $\mc V$. We make the following standing assumption on the directed graph formed by the union of graphs induced.   

\begin{assumption}
\label{ass:connectivity}
The union of the sub-graphs induced by $A^{(0)}, A^{(1)}, \ldots, A^{(m)}$ is strongly connected.
\end{assumption}

To avoid triviality, we also make the following assumption.
\begin{assumption}
\label{ass:multiplicative-uncertainty}
For all $j \in [m]$, $A^{(j)} \neq 0$, $\mu_j>0$ and $\sigma_j>0$.
\end{assumption}

\begin{example}
\label{example:linear-transportation-network}
For concreteness, let us consider the following example, adapted from \cite[Example 1]{Rantzer:15}, of a linear transportation network defined over the graph shown in Figure~\ref{fig:transportation-network-example}. This graph is the union of sub-graphs induced by $A^{(0)}$ and $A^{(1)}$ defined as follows: 
\begin{align*}
A^{(0)} & = \begin{bmatrix}
-0.1-\ell_{31} & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
\ell_{31} & 0 &  - \ell_{43} & \ell_{34} \\
0 & 0 & \ell_{43} & -\ell_{34}
\end{bmatrix} \quad
%\\
A^{(1)}  = 
\begin{bmatrix}
0 & \ell_{12} & 0 & 0 \\
0 & -\ell_{12} - \ell_{32} & \ell_{23} & 0 \\
0 & \ell_{32} & -\ell_{23} & 0 \\
0 & 0 & 0 & 0
\end{bmatrix}
\end{align*}
where $\ell_{ij} \geq 0$ for all $i, j$.

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.4\textwidth]{./fig/linear-transportation-network}
%\begin{minipage}[c]{.4\textwidth}
%\begin{center}
%\includegraphics[width=0.7\textwidth]{./fig/uncertainty-block-diagram} \\ (a)
%\end{center}
%\end{minipage}
%\hspace{0.25in}
%\begin{minipage}[c]{.4\textwidth}
%\begin{center}
%\includegraphics[width=0.9\textwidth]{./fig/MSS-feedback} \\ (b)
%\end{center}
%\end{minipage}
\end{center}
\caption{\sf A transportation network example.}
\label{fig:transportation-network-example}
\end{figure}
\end{example}

\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.4\textwidth}
\begin{center}
\includegraphics[width=0.7\textwidth]{./fig/uncertainty-block-diagram} \\ (a)
\end{center}
\end{minipage}
\hspace{0.25in}
\begin{minipage}[c]{.4\textwidth}
\begin{center}
\includegraphics[width=0.9\textwidth]{./fig/MSS-feedback} \\ (b)
\end{center}
\end{minipage}
\end{center}
\caption{\sf (a) Linear systems with both additive and multiplicative stochastic disturbances; (b) feedback interconnection used for Definition~\ref{def:MSS-feedback}.}
\label{fig:uncertainty-block-diagram}
\end{figure}

\eqref{eq:routing-discrete-time-reformulation} can be rewritten as interconnection between a structured uncertainty and a deterministic system (cf. Figure~\ref{fig:uncertainty-block-diagram}): \ksmargin{notations in Fig~\ref{fig:uncertainty-block-diagram} need to be made consistent}
\begin{equation}
\label{eq:structured-uncertainty-form}
\begin{split}
x(t+1) & = \Amatrix x(t) + B_{u} u(t) + B_w w(t) \\
y(t) & = C x(t) \\
u(t) & = \bigtriangle(t) y(t)
%u(t) & = \bar{\triangle}(t) y(t)
\end{split}
\end{equation}
Comparing \eqref{eq:routing-discrete-time-reformulation} and \eqref{eq:structured-uncertainty-form} gives:
\begin{equation}
\label{eq:state-space-matrices}
\begin{split}
\Amatrix & = I + A^{(0)} + \sum_{j=1}^m \mu_{\gamma_j} A^{(j)}, \quad B_u = [I_n \, \, I_n \, \ldots \, I_n], \quad C = [A^{(1)} \, \, A^{(2)} \, \ldots \, A^{(m)}]^T \\
\bigtriangle(t)  & = \begin{bmatrix} \triangle_1(t) \cdot I_n & & \\ & \triangle_2(t) \cdot I_n & \\ & \ldots & \\ & & \triangle_m(t) \cdot I_n \end{bmatrix}
\end{split}
\end{equation}
Corresponding to our assumption that $w(t)$ is scalar, $B_w$ is a column vector. 
%For simplicity, we assume that $w(t)$ is scalar, and accordingly $\bar{B}$ is a column vector. 

The representation~\eqref{eq:structured-uncertainty-form} can be seen as the interconnection between the structured uncertainty $\bigtriangle$ and a deterministic system $G_w$ with the following state space matrices:
\begin{equation*}
G_w: 
\left[\begin{array}{c|c|c}
\Amatrix & B_u & B_w \\
\hline
C & 0 & 0 
\end{array} \right]
\end{equation*}
We call the system seen by $\bigtriangle$ the mean system and denote it by $G$:
\begin{equation}
\label{eq:mean-system}
G: 
\left[
\begin{array}{c|c}
\Amatrix & B_u \\
\hline
C & 0
\end{array}
\right]
\end{equation}

Recall the independence assumptions on $\{\triangle_j\}_{j \in [m]}$ and $w(t)$. Accordingly, let
$$
\Sigma = \begin{bmatrix} \sigma^2_{\gamma_1} \cdot I_n & & \\ & \sigma^2_{\gamma_2} \cdot I_n & \\ & \ldots & \\ & & \sigma^2_{\gamma_m} \cdot I_n \end{bmatrix}
$$
be the covariance matrix of $\bigtriangle$. We assume that $w(t)$ has zero mean and variance $\sigma_w^2$. Our objective is to find (tight) conditions on $A^{(0)}$, $A^{(1)}, \ldots, A^{(m)}$, $\{\sigma^2_{\gamma_j}\}_{j \in [m]}$, $\Sigma$ and $\sigma_w^2$  to ensure that \eqref{eq:structured-uncertainty-form} is mean square stable. 

\begin{definition}
A causal linear time invariant system $\mathcal M$ is called \emph{Mean-Square Stable} (MSS) if for each white, second-order input process $u$ with uniformly bounded variance, the output process $y=\mathcal M u$ has uniformly bounded variance
$$
y_t := E[y_t y_t^*] \leq c \left(\sup_{\tau} \, u_{\tau} \right)
$$ 
with $c$ a constant independent of $t$ and the process $u$.
\end{definition}

\ksmargin{Definition~\ref{def:MSS-feedback} probably redundant}
The above definition is extended to feedback interconnections as follows.
\begin{definition}
\label{def:MSS-feedback}
Consider the feedback system of Figure~\ref{fig:uncertainty-block-diagram} with $d$ and $w$ being white second order processes, and $\mc M$ and $\mc G$ causal LTI systems. The feedback system in Figure~\ref{fig:uncertainty-block-diagram} is called mean-square stable if all signals $u$, $y$, $v$ and $r$ have uniformly bounded variance sequences, i.e., if there exists constant $c$ such that
$$
\max \left\{\|u\|_{\infty}, \|y\|_{\infty}, \|v\|_{\infty}, \|r\|_{\infty} \right\} \leq c \, \min \left \{\|d\|_{\infty},\|w\|_{\infty} \right \}
$$
\end{definition}




==> non-asymptotic-dynamic/instability.tex <==
\subsection{Unstable Behavior}
\label{sec:unstable} \ksmarginsoft{what implication does this have for $\Xcov(t)$?}
 %\ksmargin{Section~\ref{sec:unstable} is work in progress} 
%While Proposition~\ref{prop:stable} suggests the existence of a stochastic process $\omega(t)$ under which \eqref{eq:dynamics-non-asymptotic} is not MS stable, 
If $\rho(\Hop)>1$, which implies \eqref{eq:structured-uncertainty-form} is not MS stable, then \cite[Section VIC]{Bamieh.Filo:18} suggests that, if the additive noise $\omega(t)$ can be chosen such that $\Sigma_{\bar{\omega}}$ is equal to the \emph{Perron eigen-matrix} of $\Hop$, then \kscommentsoft{$\Ucov(t)$ grows unbounded geometrically}. 

%\input{./routing/unstable-theorem-optional}


==> non-asymptotic-dynamic/non-asymptotic-dynamic-main.tex <==
\section{Robustness of Finite Networks}
\label{sec:non-asymptotic-dynamical}
Consider the following dynamics: 
\begin{equation}
\label{eq:dynamics-non-asymptotic}
x(t+1) = \underbrace{\left( \Azero + \sum_{j \in [m]} \triangle_j(t) A^{(j)} \right)}_{=A(t)} x(t) + \omega(t)
\end{equation}
where, as before, $x(t) \in \reals^n$ denotes the states associated with the $n$ nodes of the network, $\Azero$ is the \emph{nominal} part of the dynamics, 
$\{\triangle_j(t)\}_{j \in [m]}$ are scalar-valued random processes, and $\omega(t) \in \reals^n$ is a vector-valued random process.  
%We assume that \kscomment{$\{A^{(j)}\}_{j \in [m]}$ are each of rank 1}. 
$A(t)$ in \eqref{eq:dynamics-non-asymptotic} is a special case of a general matrix-valued random process. In addition to $A$ being stochastic, \eqref{eq:dynamics-non-asymptotic} also differs from \eqref{eq:dynamics-asymptotic} in that the additive \emph{shock} in \eqref{eq:dynamics-asymptotic} is a Kronecker delta function, whereas $\omega(t)$ in \eqref{eq:dynamics-asymptotic} is a random process. 
We shall focus on random processes $\{\triangle_j(t)\}_{j \in [m]}$ and $\omega(t)$ that satisfy the following:
\begin{itemize} 
\item $\triangle(t)=[\triangle_1(t), \, \triangle_2(t), \ldots, \triangle_m(t)]^T$ is temporally independent, with $\E[\triangle(t)]=\zerobf$ and finite covariance $\Sigma_{\triangle}$
\item $\omega(t)$ is temporally independent, with $\E[\omega]=\zerobf$ and finite covariance $\Sigma_{\omega}$
\item $\triangle(t)$ and $\omega(t)$ are independent of each other, and are both independent of $\{x(\tau), \, \tau \leq t\}$
\end{itemize} 
Without loss of generality, let $\{\triangle_j\}_{j \in [m]}$ be such that $\sigma_{\triangle_j}=1$ for all $j \in [m]$. This can be done, e.g., by appropriately scaling $\{A^{(j)}\}_{j \in [m]}$. 
%Let $\Sigma_{\triangle}$ and $\Sigma_{\omega}$ be the covariance matrices of $\triangle$ and $\omega$ respectively. 
Note that the assumptions above do not preclude dependence within components of $\triangle(t)$ and $\omega(t)$ at a given $t$, i.e., $\Sigma_{\triangle}$ and $\Sigma_{\omega}$ are not assumed to be diagonal. 
Specifically, $\Sigma_{\triangle}=I$ is referred to as the case of uncorrelated uncertainties, and $\Sigma_{\triangle} \neq I$ is referred to as the case of correlated uncertainties. 

%Naturally, to avoid triviality, we assume that, for all $j \in [m]$, $A^{(j)} \neq 0$ and $\sigma_j>0$. If not, then such a $A^{(j)}$ is absorbed into $A^{(0)}$. 


%
%To avoid triviality, we also make the following assumption.
%\begin{assumption}
%\label{ass:multiplicative-uncertainty}
%For all $j \in [m]$, $A^{(j)} \neq 0$, $\mu_j>0$ and $\sigma_j>0$.
%\end{assumption}



\input{./non-asymptotic-dynamic/examples}

\input{./non-asymptotic-dynamic/stochastic-stability}

\input{./non-asymptotic-dynamic/instability}

%\input{./non-asymptotic-dynamic/flow/stochastic-uncertainty-problem-formulation}
%
%\input{./non-asymptotic-dynamic/flow/analysis}
%
%\input{./non-asymptotic-dynamic/flow/computations}

%\input{./non-asymptotic-dynamic/flow/conclusion}

==> non-asymptotic-dynamic/stochastic-stability.tex <==
\subsection{Stochastic Stability}
It is of interest to identify tight conditions on $\Azero$, $\{A^{(j)}\}_{j \in [m]}$, and statistics of $\triangle(t)$ and $\omega(t)$ under which \eqref{eq:dynamics-non-asymptotic} is mean square (MS) stable. 
%\begin{definition}
%A causal linear time invariant system $\mathcal M$ is called mean square (MS) stable if for each white, second-order input process $u$ with uniformly bounded variance, the output process $y=\mathcal M u$ has uniformly bounded variance
%$$
%\E[y^T(t) \, y(t)] \leq c \left(\sup_{\tau} \, \E[u^T(\tau) \, u(\tau)] \right)
%$$ 
%with $c$ a constant independent of $t$ and the process $u$.
%\end{definition}
%
Such a stability analysis can be performed within the classical $M-\bigtriangle$ framework (cf. Section~\ref{sec:M-Delta}) as follows. 
\eqref{eq:dynamics-non-asymptotic} can be rewritten 
%as interconnection between a \emph{structured uncertainty} and a deterministic system 
as:
\begin{equation}
\label{eq:structured-uncertainty-form}
\begin{split}
x(t+1) & = \Azero x(t) + B u(t) \\
y(t) & = C x(t) \\
r(t) & = \bigtriangle(t) y(t) \\
u(t) & = r(t) + \bar{\omega}(t)
%u(t) & = \bar{\triangle}(t) y(t)
\end{split}
\end{equation}
%\begin{equation}
%\label{eq:structured-uncertainty-form}
%\begin{split}
%x(t+1) & = A x(t) + B u(t) + B \bar{\omega}(t)\\
%y(t) & = C x(t) \\
%u(t) & = \bigtriangle(t) y(t)
%%u(t) & = \bar{\triangle}(t) y(t)
%\end{split}
%\end{equation}
%Comparing \eqref{eq:routing-discrete-time-reformulation} and \eqref{eq:structured-uncertainty-form} gives:
with   
\begin{equation}
\label{eq:state-space-matrices}
B = [\underbrace{I_n \, \, I_n \, \ldots \, I_n}_{m \text{ times}}], \quad C = \begin{bmatrix} A^{(1)} \\ A^{(2)} \\ \vdots \\ A^{(m)} \end{bmatrix}, \quad \bigtriangle(t)  = \begin{bmatrix} \triangle_1(t) \cdot I_n & & \\ & \triangle_2(t) \cdot I_n & \\ & \ldots & \\ & & \triangle_m(t) \cdot I_n \end{bmatrix}
%\begin{split}
%\Amatrix & = A^{(0)} + \sum_{j=1}^m \mu_{\gamma_j} A^{(j)}, \quad B_u = [I_n \, \, I_n \, \ldots \, I_n], \quad C = [A^{(1)} \, \, A^{(2)} \, \ldots \, A^{(m)}]^T \\
%\bigtriangle(t)  & = \begin{bmatrix} \triangle_1(t) \cdot I_n & & \\ & \triangle_2(t) \cdot I_n & \\ & \ldots & \\ & & \triangle_m(t) \cdot I_n \end{bmatrix}
%\end{split}
\end{equation}
and $\bar{\omega}(t):=\onebf_m \otimes \omega(t)$, and therefore, $\Sigma_{\bar{\omega}}=\onebf_m \onebf^T_m \otimes \Sigma_{\omega}$. 
%Corresponding to our assumption that $w(t)$ is scalar, $B_w$ is a column vector. 
%For simplicity, we assume that $w(t)$ is scalar, and accordingly $\bar{B}$ is a column vector. 
\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.4\textwidth}
\begin{center}
%\includegraphics[width=0.7\textwidth]{./fig/uncertainty-block-diagram} 
%\includegraphics[width=1.0\textwidth]{./fig/MSS-feedback} 
\includestandalone[width=0.8\linewidth]{./fig/M-Delta}
%\\ (a)
\end{center}
\end{minipage}
%\hspace{0.25in}
%\begin{minipage}[c]{.4\textwidth}
%\begin{center}
%\includegraphics[width=0.9\textwidth]{./fig/MSS-feedback} \\ (b)
%\end{center}
%\end{minipage}
\end{center}
\caption{\sf The strictly causal LTI system $\mc M$ in \eqref{eq:G-def} in feedback with multiplicative stochastic gain $\bigtriangle$ in \eqref{eq:state-space-matrices}. 
%(b) feedback interconnection used for Definition~\ref{def:MSS-feedback}.
}
\label{fig:uncertainty-block-diagram}
\end{figure}

The representation~\eqref{eq:structured-uncertainty-form} can be seen as the interconnection between structured uncertainty $\bigtriangle$ and a deterministic system $\mc M$ with the following state space matrices (see Figure~\ref{fig:uncertainty-block-diagram}): 
\begin{equation}
\label{eq:G-def}
%\mc M_{\omega}: 
%\left[\begin{array}{c|c|c}
%A & B & B \\
%\hline
%C & 0 & 0 
%\end{array} \right]
%, \quad 
\mc M: 
\left[
\begin{array}{c|c}
\Azero & B \\
\hline
C & 0
\end{array}
\right]
\end{equation}
%where $\mc M$ is the \emph{mean system} seen by $\bigtriangle$.
%\begin{equation}
%\label{eq:mean-system}
%G: 
%\left[
%\begin{array}{c|c}
%\Amatrix & B_u \\
%\hline
%C & 0
%\end{array}
%\right]
%\end{equation}

%
%
%
%Recall the independence assumptions on $\{\triangle_j\}_{j \in [m]}$ and $w(t)$. Accordingly, let
%$$
%\Sigma = \begin{bmatrix} \sigma^2_{\gamma_1} \cdot I_n & & \\ & \sigma^2_{\gamma_2} \cdot I_n & \\ & \ldots & \\ & & \sigma^2_{\gamma_m} \cdot I_n \end{bmatrix}
%$$
%be the covariance matrix of $\bigtriangle$. 
%We assume that $w(t)$ has zero mean and variance $\sigma_w^2$. Our objective is to find (tight) conditions on $A^{(0)}$, $A^{(1)}, \ldots, A^{(m)}$, $\{\sigma^2_{\gamma_j}\}_{j \in [m]}$, $\Sigma$ and $\sigma_w^2$  to ensure that \eqref{eq:structured-uncertainty-form} is mean square stable. 



%\ksmargin{Definition~\ref{def:MSS-feedback} probably redundant}
%The above definition is extended to feedback interconnections as follows.
\begin{definition}
\label{def:MSS-feedback}
The feedback system in \eqref{eq:structured-uncertainty-form} is called mean-square (MS) stable if signals $y$ and $r$ have uniformly bounded variance sequences, i.e., if there exists a constant $c$ such that
$$
\max \left\{ \|\E[y(t)y^T(t)]\|_{\infty}, \|\E[r(t)r^T(t)]\|_{\infty} \right\} \leq c 
$$
\end{definition}

%The next result is an adaptation of Theorem 3.2 and Section VI in \cite{Bamieh.Filo:18}. 

The next result gives a tight condition on MS stability of \eqref{eq:structured-uncertainty-form}. 
\begin{theorem}
\label{thm:stable-main}
Let $\rho(\Azero)<1$. \eqref{eq:structured-uncertainty-form} is MS stable if and only if $\rho(\Hop)<1$, where
the matrix-valued linear operator $\map{\Hop}{\reals^{nm \times nm}}{\reals^{nm \times nm}}$, also known as the \emph{loop gain operator}, is defined as:
\begin{equation}
\label{eq:H-def}
\begin{split}
\Hop(\bar{X}) :=\Sigma_{\bar{\bigtriangle}} \circ \left(\sum_{t=0}^{\infty} C {\Azero}^{t} B \bar{X} B^T {{\Azero}^T}^{t}C^T \right)
\end{split}
\end{equation}
where $\Sigma_{\bar{\bigtriangle}}=\Sigma_{\triangle} \otimes \onebf_n \onebf_n^T$.
\end{theorem}

%\begin{theorem}
%\label{thm:stable-main} \ksmargin{is $\rho(A)<1$ redundant?}
%Let \kscomment{$\rho(\Azero)<1$}. \eqref{eq:structured-uncertainty-form} is MS stable if and only if either of the following conditions hold:
%\begin{enumerate}
%\item[(a)] $\exists \, X > 0$ such that $\Hop(X)< X$, where 
%\begin{equation}
%\label{eq:H-def}
%\Hop(X):=\Azero X {\Azero}^T + \sum_{j, k \in [m]} \Sigma_{\triangle,jk} A^{(j)} X {A^{(k)}}^T
%\end{equation}
%\item[(b)] $\rho(\Hop)<1$
%\item[(c)] the following LMI has a solution $X \geq 0$ for some $\lambda<1$:
%\begin{equation}
%\label{eq:LMI}
%\lambda \left(X - \Azero X {\Azero}^T \right) - \sum_{j,k \in [m]} \Sigma_{\triangle,jk} A^{(j)} X {A^{(k)}}^T = 0 
%\end{equation}
%\end{enumerate}
%\end{theorem}
Theorem~\ref{thm:stable-main} is a simple application of \cite[Theorem 3.2]{Bamieh.Filo:18}, by writing the input-output form of the system $\mc M$ in \eqref{eq:G-def} (assuming zero initial condition) as:
$$
y(t) = \sum_{\tau=0}^t C {\Azero}^{t-\tau-1} B u_{\tau}
$$
%\cite{Wang.Elia:12} provides a result similar to Theorem~\ref{thm:stable-main} for the special case of uncorrelated uncertainties, i.e., $\Sigma_{\triangle}=I$, for distributed averaging dynamics.
%
% 
%\begin{proposition}
%\label{prop:stable-main-uncorrelated}
%Let \kscomment{$\rho(A)<1$}, and $\Sigma_{\triangle}=I$. \eqref{eq:structured-uncertainty-form} is MS stable if and only if either of the following conditions hold:
%\begin{enumerate}
%\item[(a)] $\exists \, X > 0$ such that $\mathbb{H}(X)< X$, where 
%\begin{equation}
%\label{eq:H-def}
%\mathbb{H}(X):=A X A^T + \sum_{j=1}^m A^{(j)} X {A^{(j)}}^T
%\end{equation}
%\item[(b)] $\rho(\mathbb{H})<1$
%%\begin{equation}
%%\label{eq:spectral-radius-condition}
%%\rho(\mc H)<1
%%\end{equation}
%%
%%$\rho(\mc H)<1$, where
%%$$
%%\mc H:=AXA^T + \sum_i \sigma_i^2 B(i) C_i X C_i^T B^T(i)
%%$$
%%\item[(c)] The mean system $G$ is stable (cf Definition~\eqref{eq:mean-system}) and satisfies $\rho(\|G\|_2^2 \Sigma)<1$
%%where 
%%$$
%%\|G\|_2^2 = \begin{bmatrix}
%%\|G_{11}\|_2^2 & \ldots & \|G_{1m}\|_2^2 \\
%%\vdots & \ldots & \vdots \\
%%\|G_{m1}\|_2^2 & \ldots & \|G_{mm}\|_2^2
%%\end{bmatrix}
%%$$
%%and $\Sigma$ is the covariance matrix of $\bigtriangle$.
%\end{enumerate}
%\end{proposition}
%Proposition~\ref{prop:stable-main-uncorrelated} follows from \cite[Theorem 1]{Wang.Elia:12}, and its proof is provided in Section~\ref{sec:stable-main-uncorrelated} for completeness. 
\cite[Section IVA]{Bamieh.Filo:18} establishes that $\rho(\|\mc M\|_2^2)<1$ is also a necessary and sufficient condition for MS stability of \eqref{eq:structured-uncertainty-form} when $\Sigma_{\triangle}=I$ (uncorrelated uncertainties), where $\|\mc M\|_2^2$ is the matrix of squared $\mc H^2$ norms of subsystems of $\mc M$ in \eqref{eq:G-def}. However, for correlated uncertainties, i.e., $\Sigma_{\triangle} \neq I$, \cite[Section IVC]{Bamieh.Filo:18} argues that such a condition involving only $\mc H^2$ norms of subsystems is not enough, and that one needs in addition other system metrics, like the inner product between different subsystems' impulse responses. 

For distributed averaging dynamics, all rows sums of $\Azero$ are equal to one, and, indeed $\rho(\Azero)=1$. While Theorem~\ref{thm:stable-main} does not apply directly, \cite{Wang.Elia:12} provides a  decomposition of the state into the \emph{conserved} state and the \emph{deviation} state. The dynamics of the deviation state is decoupled from that of the conserved state, and moreover the spectral radius of its nominal dynamics is less than 1, and therefore amenable to Theorem~\ref{thm:stable-main}.

Computationally, \cite[Section VI]{Bamieh.Filo:18} suggests that $\rho(\Hop)$ is the largest real number $\lambda$ such that the following LMI has a feasible solution $X \geq 0$:
\begin{equation*}
\label{eq:LMI}
\lambda \left(X - \Azero \bar{X} {\Azero}^T \right) - B \left(\Sigma_{\bar{\bigtriangle}} \circ (C \bar{X} C^T)\right) B^T = 0 
\end{equation*}
which, by plugging in \eqref{eq:state-space-matrices}, can be rewritten as:
$$
\lambda \left(\bar{X} - \Azero \bar{X} {\Azero}^T \right) - \sum_{j,k \in [m]} \Sigma_{\triangle,jk} A^{(j)} \bar{X} {A^{(k)}}^T = 0
$$

It is instructive to look at the \emph{covariance feedback system}~\cite{Bamieh.Filo:18} associated with \eqref{eq:dynamics-non-asymptotic}:
\begin{align*}
\Xcov(t+1) & = \Azero \Xcov(t) {\Azero}^T + B \Ucov(t) B^T \\
\Ycov(t) & = C \Xcov(t) C^T \\
\Ucov(t) & = \Sigma_{\bar{\bigtriangle}} \circ \Ycov(t) + \Sigma_{\bar{\omega}}
\end{align*}
from which boundedness of $\Ycov(t)$ and hence also of $\Ucov(t)$, when \eqref{eq:structured-uncertainty-form} is MS stable, implies boundedness of $\Xcov(t)$. In the noiseless case, i.e., $\Sigma_{\bar{\omega}}=\zerobf$, it can be argued that $\Xcov(t) \to \zerobf$.

%\kscomment{
%If $\Sigma_{\omega}=\zerobf$, i.e., no additive noise, then MS stability of \eqref{eq:structured-uncertainty-form} implies that $x(t) \to \zerobf$ almost surely, and $\E[x(t)] \to \zerobf$. The converse is established as follows.
%
%%\begin{definition}
%%\eqref{eq:structured-uncertainty-form} is said to be MS \kscomment{convergent} if, under $w(t) \equiv 0$, $E x(t) \to 0$. 
%%\end{definition}
%
%\begin{proposition}
%\label{prop:stable}
%Let $\Sigma_{\omega}=\zerobf$. $\E[x(t)] \to \zerobf$ if and only if \eqref{eq:structured-uncertainty-form} is MS stable. 
%\end{proposition}
%}


%The following procedure is adapted from \cite{Bamieh.Filo:18}. To calculate the spectral radius of $\mc H$ defined in \eqref{eq:H-def}, one can find the largest real number $\lambda$ which satisfies the following 
%\begin{equation*}
%\label{eq:LMI}
%\begin{split}
%\lambda \left(X - A X A^T \right) - \sum_{j=1}^m \sigma^2_{\triangle_j} A^{(j)} X {A^{(j)}}^T & = 0 
%\\
%X & \geq 0
%\end{split}
%\end{equation*}


==> routing/analysis.tex <==
\section{Analysis}
The results in this section are inspired by \cite{Wang.Elia:12}.

\begin{theorem}
\label{thm:stable-main}
\eqref{eq:structured-uncertainty-form} is MS stable, if and only if either of the following conditions hold:
\begin{enumerate}
\item[(a)] $\exists \, X > 0$ such that $\mc H (X)< X$, where 
\begin{equation}
\label{eq:H-def}
\mc H(X):=\Amatrix X \Amatrix^T + \sum_{j=1}^m \sigma^2_{\gamma_j} A^{(j)} X {A^{(j)}}^T
\end{equation}
\item[(b)] $\rho(\mc H)<1$
%\begin{equation}
%\label{eq:spectral-radius-condition}
%\rho(\mc H)<1
%\end{equation}
%
%$\rho(\mc H)<1$, where
%$$
%\mc H:=AXA^T + \sum_i \sigma_i^2 B(i) C_i X C_i^T B^T(i)
%$$
%\item[(c)] The mean system $G$ is stable (cf Definition~\eqref{eq:mean-system}) and satisfies $\rho(\|G\|_2^2 \Sigma)<1$
%where 
%$$
%\|G\|_2^2 = \begin{bmatrix}
%\|G_{11}\|_2^2 & \ldots & \|G_{1m}\|_2^2 \\
%\vdots & \ldots & \vdots \\
%\|G_{m1}\|_2^2 & \ldots & \|G_{mm}\|_2^2
%\end{bmatrix}
%$$
%and $\Sigma$ is the covariance matrix of $\bigtriangle$.
\end{enumerate}
\end{theorem}

\ksmargin{can we get rid of $\sigma_w=0$?}
\kscomment{
If $\sigma_w=0$}, then MS stability implies that $x(t) \to 0 $ almost surely, and $E[x(t)] \to 0$. The converse is established as follows.

%\begin{definition}
%\eqref{eq:structured-uncertainty-form} is said to be MS \kscomment{convergent} if, under $w(t) \equiv 0$, $E x(t) \to 0$. 
%\end{definition}

\begin{proposition}
\label{prop:stable}
Consider \eqref{eq:structured-uncertainty-form} with $\sigma_w=0$. $E[x(t)] \to 0$ if and only if \eqref{eq:structured-uncertainty-form} is MS stable. 
\end{proposition}

The next result gives further insight into the behavior when \eqref{eq:structured-uncertainty-form} is MS unstable.



\begin{theorem}
\label{thm:unstable}
Let Assumption~\ref{ass:connectivity} hold true. If \eqref{eq:structured-uncertainty-form} is MS unstable, then $\lim_{t \to \infty} E[(x_i(t)-x_i(t-1))^2] = \infty$ for all $i \in \mc V$.
%The following results hold true.
%\begin{enumerate} 
%\item[(a)] 
%$\lim_{t \to \infty} E[x_i(t)] = \infty$ and 
%\item[(b)] Let \kscomment{$\eta < 0$}. \kscomment{$x_i(t)$ (or $x_i(t)-x_i(t-1)$?)} converges in distribution to a random variable $R_i$, for all $i \in \mc V$, as $t \to \infty$. Furthermore, $R_i$ has unbounded second moment if and only if \eqref{eq:structured-uncertainty-form} is MS unstable.
%\end{enumerate}
\end{theorem}



==> routing/computations.tex <==
\section{Computations}
The following procedure is adapted from \cite{Bamieh.Filo:18}. To calculate the spectral radius of $\mc H$ defined in \eqref{eq:H-def}, one can find the largest real number $\lambda$ which satisfies the following 
\begin{equation*}
\label{eq:LMI}
\begin{split}
\lambda \left(X - \Amatrix X \Amatrix^T \right) - \sum_{j=1}^m \sigma^2_{\gamma_j} A^{(j)} X {A^{(j)}}^T & = 0 
\\
X & \geq 0
\end{split}
\end{equation*}

==> routing/conclusion.tex <==
\section{Future Work}
Extensions to:
\begin{enumerate}
\item non-diagonal $\bigtriangle$
\item non-linear network flow dynamics in \cite{Como.Savla.ea:Part1TAC10} and \cite{Como.Lovisari.ea:TCNS13}
\item vector $w(t)$
\item $w(t)$ as non-negative r.v.
\item enforce non-negativity on $x(t)$
\end{enumerate}

==> routing/proofs-old.tex <==
\subsection{Proof of Theorem~\ref{thm:stable-main}}
\label{sec:stable-main-uncorrelated}
The input-output form of the system $\mc M$ in \eqref{eq:G-def} (assuming zero initial condition) is: 
$$
y(t) = \sum_{\tau=0}^t C {\Azero}^{t-\tau-1} B u_{\tau}
$$
The theorem then follows from \cite[Theorem 3.2]{Bamieh.Filo:18}.
% implies that \eqref{eq:structured-uncertainty-form} is MS stable if and only if the spectral radius of the following operator is less than 1: $\Sigma_{\bar{\bigtriangle}} \circ \left(\sum_{t=0}^{\infty} C {\Azero}^{t} B X B^T {{\Azero}^T}^{t}C^T \right)$, where $\Sigma_{\bar{\bigtriangle}}=\Sigma_{\triangle} \otimes \onebf_n \onebf_n^T$. Plugging in the values from \eqref{eq:state-space-matrices} gives \eqref{eq:H-def}.

%\subsection{Proof of Theorem~\ref{thm:stable-main}}
%%\begin{proof}
%\eqref{eq:structured-uncertainty-form} can be re-written compactly as:
%$$
%x(t+1) = \Azero x(t) + B \bigtriangle(t) C x(t)+ B \bar{\omega}(t)
%$$
%Therefore,
%\begin{equation}
%\label{eq:var-expr}
%\begin{split}
%\E[x(t+1)x(t+1)^T] = & \Azero \E[x(t)x(t)^T]{\Azero}^T + \E[B \bigtriangle(t) C x(t) x(t)^T {\Azero}^T] \\
%& + \E[\Azero x(t) x(t)^T C^T \bigtriangle(t) B^T] + \E[B \bigtriangle(t) C x(t) x(t)^T C^T \bigtriangle(t) B^T] \\
%& + B \Sigma_{\bar{\omega}} B^T
%\end{split}
%\end{equation}
%where we have used the independence assumption between $\bar{\omega}(t)$, $\bigtriangle(t)$, and $x(t)$. Let $\bar{X}(t):=\E[x(t)x(t)^T]$ denote the state correlation matrix. Using the independence assumption between $x(t)$ and $\bigtriangle$, and simple algebra, \eqref{eq:var-expr} can be rewritten as 
%\begin{equation}
%\label{eq:state-correlation}
%\begin{split}
%\bar{X}(t+1) = \Azero \bar{X}(t) {\Azero}^T + \sum_{j, k \in [m]} \Sigma_{\triangle,jk} A^{(j)} \bar{X}(t) {A^{(k)}}^T + B \Sigma_{\bar{\omega}} B^T
%\end{split}
%\end{equation}
%\ksmargin{complete}
%\kscomment{For the $\Sigma_{\omega}=\zerobf$ (no additive noise), and hence $\Sigma_{\bar{\omega}}=\zerobf$ case, \cite[Chapter 9]{Boyd.ElGhaoui.ea:94} implies (a). The equivalence between (a) and (b) is known from \cite[Proposition 2.6]{Costa.Fragoso.ea:06}. (c) follows from Theorem 3.2 and Section VI in \cite{Bamieh.Filo:18}.} 
%%The equivalence between (a) and (c) follows from \cite[Theorem 6.4]{Elia:05}.
%%where we have assumed that, at a given $t$, $\gamma_i(t)$ is independent of $\{\gamma_j(t), \, j \in [n] \setminus \{i\}\}$.
%%\end{proof}

%\subsection{Proof of Proposition~\ref{prop:stable}}
%%\begin{proof}
%\ksmargin{check the proof}
%Sufficiency is easy to argue. Necessity follows from the application of Cauchy-Schwarz inequality:
%$
%|\E x_i(t) x_j(t)| \leq \sqrt{\E x_i^2(t) E x_j^2(t)}
%$.
%%\end{proof}

\subsection{A Technical Lemma}
\begin{lemma}
\label{lem:unstable}
Let the conditions of Theorem~\ref{thm:unstable} hold true. If \eqref{eq:structured-uncertainty-form} is not MS stable, then 
$$
\lim_{t \to \infty} \E \left(\Abar_i x(t) x^T(t) \Abar_{i}^T \right) = \infty, \qquad \forall \, i \in [n]$$
where $\Abar:=\sum_{j=0}^m \tilde{A}^{(j)}-I$.
\end{lemma}
\begin{proof} 
Let $M_1$ be the eigenvector of $\Hop$ (cf. \eqref{eq:H-def}) associated with the eigenvalue of largest magnitude, say $\lambda$. \kscomment{Along the lines of the proof of \cite[Lemma 4]{Wang.Elia:12}, we first show that $M_1 \geq 0$ and $\lambda \geq 1$}, with: \ksmargin{This part may follow simply from \cite[Theorem 2.3]{Bamieh.Filo:18}}
\begin{equation}
\label{eq:H-eigen-equation}
\lambda M_1 = \Azero M_1 {\Azero}^T + \sum_{j \in [m]} A^{(j)} M_1 {A^{(j)}}^T = \Hop(M_1)
\end{equation}

Recall that the state correlation matrix $\bar{X}=\E[xx^T]$ satisfies the following update \kscomment{(for $\Sigma_{\omega}=\zerobf$)}: $X(t+1) = \Hop(X(t))$ (cf. \eqref{eq:state-correlation}). Consider the following re-scaled version of this update rule: 
\begin{equation}
\label{eq:correlation-update-rescaled}
X(t+1) = \Hop_{\lambda}(X(t)):=\frac{1}{|\lambda|}\Hop(X(t))
\end{equation}
%
%Re-scaling the right hand side of \eqref{eq:state-correlation} for \kscomment{$\sigma_w=0$} by \kscomment{$\rho(\mc H)=|\lambda|$}, we get 
%$$
%\tilde{X}(t+1) = \frac{1}{|\lambda|}\Amatrix \tilde{X}(t) \Amatrix^T + \frac{1}{|\lambda|} \sum_{j=1}^m \sigma^2_{\gamma_j} A^{(j)} \tilde{X}(t) {A^{(j)}}^T 
%$$
$\rho(\Hop) \geq 1$ implies $\rho(\Hop_{\lambda})=1$. Therefore, \eqref{eq:correlation-update-rescaled} is not MS stable, and \cite[Chapter 9]{Boyd.ElGhaoui.ea:94} then implies that the following LMI is infeasible:
$$
\mc F(X):=
\begin{bmatrix}
X & 0 \\
0 & -\Hop_{\lambda}^*(X) + X
\end{bmatrix} > 0
$$
where $\Hop^*_{\lambda}(X):=\frac{1}{|\lambda|}{\Azero}^T X \Azero + \frac{1}{|\lambda|}\sum_{j \in [m]}  {A^{(j)}}^T X A^{(j)}$ is the adjoint of $\Hop_{\lambda}$. 
%$$
%X>0, \, \frac{1}{|\lambda|}\Amatrix \tilde{X}(t) \Amatrix^T + \frac{1}{|\lambda|} \sum_{j=1}^m \sigma^2_{\gamma_j} A^{(j)} \tilde{X}(t) {A^{(j)}}^T - X < 0
%$$
%The second LMI can be written as $\mc H^*(X)/|\lambda| - X<0$, where $\mc H^*:=\Amatrix^T X \Amatrix + \sum_{j=1}^m \sigma^2_{\gamma_j} {A^{(j)}}^T X A^{(j)}$ is the adjoint of $\mc H$. 
Duality theory then implies that there exists a positive semi-definite matrix $J$ such that $\Tr(J \mc F_i)=0$ for $i = 1, \ldots, \bar{n}:=n(n+1)/2$, where $\{\mc F_i\}_{i=1}^{\bar{n}}$ is a base for $\mc F(X)$. If $\{P_i\}_{i=1}^{\bar{n}}$ denotes the base for all symmetric matrices, then 
$$
\mc F_i = \begin{bmatrix}
P_i & 0 \\
0 & -\Hop_{\lambda}^*(P_i) + P_i 
\end{bmatrix}
$$
and, hence, 
$$
\Tr \left\{ 
\begin{bmatrix}
P_i & 0 \\ 
0 & - \Hop^*_{\lambda}(P_i) + P_i
\end{bmatrix} \cdot 
\begin{bmatrix}
J_{11} & J_{12} \\
J_{21} & J_{22}
\end{bmatrix}
\right\} = 0
$$ 
which is equivalent to
\begin{equation}
\label{eq:trace}
\Tr\left\{P_i \left(J_{11} - \Hop_{\lambda}(J_{22}) + J_{22} \right) \right\} = 0
\end{equation}
Since $\{P_i\}_{i=1}^{\bar{n}}$ form the basis of symmetric matrices, \eqref{eq:trace} implies that, for any $x \in \reals^n$,  
$$
\Tr \left\{x x^T (J_{11} - \Hop_{\lambda}(J_{22}) + J_{22}) \right\} =0
$$
and, hence, 
$$
x^T \left(J_{11} - \Hop_{\lambda}(J_{22}) + J_{22} \right) x = 0
$$
which implies that $J_{22} \leq \Hop_{\lambda}(J_{22})$. $J$ is positive semidefinite and therefore so are $J_{11}$ and $J_{22}$. Therefore, using the definition of $\Hop_{\lambda}$, we get
\begin{equation}
\label{eq:eigen-subequation}
|\lambda| J_{22} \leq \Hop(J_{22})
\end{equation}
Since $\lambda$ is the eigenvalue of $\Hop$ that has the largest magnitude, \eqref{eq:eigen-subequation} holds with equality, and hence $M_1=J_{22} \geq 0$  is the eigenvector of $\Hop$ with the eigenvalue $|\lambda|$.

Having established \eqref{eq:H-eigen-equation}, we now show the lemma through contradiction. Pick an arbitrary $i \in [n]$, and suppose, by contradiction, that $\Abar_{i} M_1 \Abar_{i}^T=0$. Multiplying by $\Abar_{i}$ and $\Abar^T_{i}$ on both sides of \eqref{eq:H-eigen-equation}, we get 
\begin{equation}
\label{eq:H-eigen-equation-1}
\Abar_{i} \Hop(M_1) \Abar_{i}^T = \Abar_{i} \Azero M_1 {\Azero}^T \Abar^T_{i} + \sum_{j \in [m]}  \Abar_{i} A^{(j)} M_1 {A^{(j)}}^T \Abar_{i} = \lambda \Abar_{i} M_1 \Abar^T_{i} = 0
\end{equation}
$M_1 \geq 0$ implies $\Azero M_1 {\Azero}^T \geq 0$ and $A^{(j)} M_1 {A^{(j)}}^T \geq 0$ for all $j \in [m]$. 
Therefore, \eqref{eq:H-eigen-equation-1} implies that  $\Abar_{i} \Azero M_1 {\Azero}^T \Abar^T_{i}=0$ and $\Abar_{i} A^{(j)} M_1 {A^{(j)}}^T \Abar_{i}=0$ for all $j \in [m]$. Repeatedly multiplying \eqref{eq:H-eigen-equation} by $\Azero$ on the left and by ${\Azero}^T$ on the right and then multiplying by $\Abar_{i}$ on the left and by $\Abar^T_{i}$ on the right, we get $\Abar_{i} (\Azero)^p M_1 ({\Azero}^T)^p \Abar^T_{i}=0$ and $\Abar_{i} (\Azero)^p A^{(j)} M_1 {A^{(j)}}^T({\Azero}^T)^p \Abar^T_{i}=0$ for all $p \geq 0$ and $j \in [m]$. This in turn implies that $M_1 ({\Azero}^T)^p \Abar^T_{i}=0$ and 
\begin{equation}
\label{eq:evalue-zero}
M_1 {A^{(j)}}^T({\Azero}^T)^p \Abar^T_{i}=0, \quad \forall p \geq 0, \,  j \in [m] 
\end{equation}

We next show that there exists at least one $j \in [m]$ such that $M_1 {A^{(j)}}^T \neq 0$. Suppose, by contradiction, that no such $j$ exists. \kscommentsoft{Then, the transfer function seen by $\bigtriangle$ is zero and the system without noise is purely deterministic. In other words, we must have the transfer function $C \left(zI-A \right)^{-1} B = 0$}, and hence $CB=0$, which, from \eqref{eq:state-space-matrices}, implies the contradiction that $A^{(j)}=0$ for all $j \in [m]$. Therefore, $M_1 {A^{(j)}}^T \neq 0$ for some $j \in [m]$, and hence \eqref{eq:evalue-zero} implies:
\begin{equation}
\label{eq:postulate}
\Abar_{i} {\Azero}^p = 0, \qquad \forall \, p \geq 0
\end{equation}

We now show that \eqref{eq:postulate} can not hold true. 
If all the elements of $\Abar_{i}$ are nonzero, we get a contradiction with \eqref{eq:postulate} for $p=0$. 
Let $\Abar_{ik}=0$ for some $k \in [n]$. \eqref{eq:diag-entries} implies that $k \neq i$. $\Abar_{ik}=0$ for $k \neq i$ implies that there is no arc between $i$ and $k$. We next exploit the structure of $\Abar_{i} {\Azero}^p$ to show that \eqref{eq:postulate} is not true. 
%First recall that $\Amatrix=I_n + A_0 + \sum_{j \in [m]} \mu_{\gamma_j} A_j$. 
%\kscomment{
%Therefore, we have that 
%\begin{align*}
%A_{0,i} \Amatrix & = A_{0,i} + A_{0,i} A_0 + \sum_{j \in [m]} \mu_{\gamma_j} A_{0,i} A_j \\
%& = A_{0,i} + 
%\end{align*}
%}
Recall $\Abar = \sum_{j=0}^m \tilde{A}^{(j)} - I=:\tilde{A}-I$. Therefore,
\begin{equation}
\label{eq:interim-1}
\Abar_i \Azero(k) = \left(\tilde{A}_i - e_i^T \right)\Azero(k) = \tilde{A}_i \Azero(k) - \Azero_{ik} = \sum_{\ell \in [n]} \tilde{A}_{i\ell} \Azero_{\ell k} - \Azero_{ik}
\end{equation}
%
%\begin{equation}
%\label{eq:A-product}
%\Abar_i \Azero = \bar{\Amatrix}_i + \bar{\Amatrix}_i \bar{\Amatrix} = \bar{\Amatrix}_i + \bar{a}_{ii} \bar{\Amatrix}_i + \sum_{j \in N_i} \bar{a}_{ij} \bar{\Amatrix}_j = \left(1+ \bar{a}_{ii}\right) \bar{\Amatrix}_i + \sum_{j \in N_i} \bar{a}_{ij} \bar{\Amatrix}_j
%\end{equation}
%where $N_i$ is the set of neighbors of $i$. 
%Note that $\bar{a}_{ij}>0$ for all $j \in N_i$, and $\bar{a}_{ii}<0$. 
The assumption that all the off-diagonal entries of $\{\tilde{A}^{(j)}\}_{j=0}^m$ have the same sign implies and that $\{\mu_j\}_{j \in [m]}$ are all positive implies that the signs of the off-diagonal entries of $\Azero$ and $\tilde{A}$ are the same. Therefore, $\Abar_{ik}=0$ implies $\Azero_{ik}=0$. Combining all these implies that the second time on the right hand side of \eqref{eq:interim-1} is zero and each entry inside the summation in the first term is non-negative. If there is an $\ell \notin \{i,k\}$ such that $\tilde{A}_{i\ell} \neq 0$ and $\Azero_{\ell k} \neq 0$ (i.e., there is a path of length 2 between $i$ and $k$), then $\Abar_i \Azero(k)>0$ contradicting \eqref{eq:postulate}. If there is no such $\ell$, then it also implies that $\sum_{\ell \in [n]} \Azero_{i \ell} \Azero_{\ell k}=(\Azero)^2_{ik}=0$. Therefore, 
$$
\Abar_i (\Azero)^2(k) = \sum_{\ell \in [n]} \tilde{A}_{i \ell} (\Azero)^2_{\ell k} - (\Azero)^2_{ik} = \sum_{\ell \in [n]} \tilde{A}_{i \ell} (\Azero)^2_{\ell k}
$$
One can argue similarly as before that each entry in the summation has the same sign as the off-diagonal entries and that it is not zero if and only if there exists an $\ell$ such that $\tilde{A}_{i\ell} \neq 0$ and $(\Azero)^2_{\ell k} \neq 0$ (i.e., there is a path of length 3 between $i$ and $k$). If this is not the case, then one can continue with the argument until the strong connectivity assumption implies that $\bar{A}_i (\Azero)^{\tilde{p}}(k)=0$ for some $\tilde{p}$, contradicting \eqref{eq:postulate}.
%Either, there is an arc from $k$ to a $j \in N_i$, or there is not. In the first case, the $k$-th component of the first term in \eqref{eq:A-product} is zero by assumption, whereas the $k$-th component of the second term is positive. Therefore, the $k$-th component of $\bar{\mc A}_1 \mc A$ is positive. 
%
%Thus, some of the zero components of $\bar{\mc A}_i$ correspond to nonzero components of $\bar{\mc A}_i \mc A$. More precisely, these are all the nodes connected to $i$ by a path of length two. In general, following Assumption~\ref{ass:connectivity}, if the $\bar{\mc A}_{ik}=0$, then there exist some $j$ for which the $k$-th component of $\bar{\mc A}_i \mc A^j$ is not zero, thereby contradicting \eqref{eq:postulate}. 
\end{proof}

\subsection{Proof of Theorem~\ref{thm:unstable}}
\label{sec:unstable-proof}
%\begin{proof}
%\begin{enumerate}
%\item[(a)] 
For $\Gamma(t)=\onebf$, \eqref{eq:dynamics-original} becomes $x(t+1)=\sum_{j=0}^m \tilde{A}^{(j)} x(t) + \omega(t)$, and therefore, 
\begin{equation*}
\label{eq:Abar-def}
x(t+1)-x(t)=(\underbrace{\sum_{j=0}^m \tilde{A}^{(j)}-I}_{\Abar}) \, x(t) + \omega(t)
\end{equation*}
Without loss of generality, we provide proof only for $i=1$; the result for other states follow similarly. 
%The iteration for $x_1$ is given by:
%$$
%x_1(t+1)-x_1(t) = \bar{\Amatrix}_{1} x(t) + B_{w,1} w(t)
%$$
%where $\bar{\Amatrix}:=\Amatrix - I_n$. 
When $\Gamma(t)=\onebf$, $x_1(t+1)-x_1(t)=\Abar_1 x(t) + \omega_1(t)$ (recall that $\Abar_1$ denotes the first row of $\Abar$), which, using the independence of $x(t)$ and $\omega(t)$, implies $\left(x_1(t+1) - x_1(t) \right)^2=\Abar_{1} x(t) x^T(t) \Abar_{1}^T + \Sigma_{\omega,11} \geq \Abar_{1} x(t) x^T(t) \Abar_{1}^T=\left(\Abar_{1} x(t)\right)^2 \geq 0$. $\left(x_1(t+1) - x_1(t) \right)^2$ can be similarly shown to be non-negative for other realizations of $\Gamma(t)$. Therefore, 
$$
\E[\left(x_1(t+1) - x_1(t) \right)^2] \geq \Pr(\Gamma=\onebf) \cdot \E [\Abar_{1} x(t) x^T(t) \Abar_{1}^T ], \qquad \forall \, t \geq 0  
$$
which, using Lemma~\ref{lem:unstable}, implies 
%Thus, \kscomment{if \eqref{eq:structured-uncertainty-form} is MS unstable, then $\lim_{t \to \infty} E \left((A_0)_1 x(t) x^T(t) (A_0)_1^T \right) = \infty$}, and hence, 
$\lim_{t \to \infty} \E[(x_1(t)-x_1(t-1))^2] = \infty$.
%\item[(b)]
%\end{enumerate}
%\end{proof}

==> routing/proofs.tex <==
%\subsection{Proof of Theorem~\ref{thm:stable-main}}
%\label{sec:stable-main-uncorrelated}
%The input-output form of the system $\mc M$ in \eqref{eq:G-def} (assuming zero initial condition) is: 
%$$
%y(t) = \sum_{\tau=0}^t C {\Azero}^{t-\tau-1} B u_{\tau}
%$$
%The theorem then follows from \cite[Theorem 3.2]{Bamieh.Filo:18}.
% implies that \eqref{eq:structured-uncertainty-form} is MS stable if and only if the spectral radius of the following operator is less than 1: $\Sigma_{\bar{\bigtriangle}} \circ \left(\sum_{t=0}^{\infty} C {\Azero}^{t} B X B^T {{\Azero}^T}^{t}C^T \right)$, where $\Sigma_{\bar{\bigtriangle}}=\Sigma_{\triangle} \otimes \onebf_n \onebf_n^T$. Plugging in the values from \eqref{eq:state-space-matrices} gives \eqref{eq:H-def}.

%\subsection{Proof of Theorem~\ref{thm:stable-main}}
%%\begin{proof}
%\eqref{eq:structured-uncertainty-form} can be re-written compactly as:
%$$
%x(t+1) = \Azero x(t) + B \bigtriangle(t) C x(t)+ B \bar{\omega}(t)
%$$
%Therefore,
%\begin{equation}
%\label{eq:var-expr}
%\begin{split}
%\E[x(t+1)x(t+1)^T] = & \Azero \E[x(t)x(t)^T]{\Azero}^T + \E[B \bigtriangle(t) C x(t) x(t)^T {\Azero}^T] \\
%& + \E[\Azero x(t) x(t)^T C^T \bigtriangle(t) B^T] + \E[B \bigtriangle(t) C x(t) x(t)^T C^T \bigtriangle(t) B^T] \\
%& + B \Sigma_{\bar{\omega}} B^T
%\end{split}
%\end{equation}
%where we have used the independence assumption between $\bar{\omega}(t)$, $\bigtriangle(t)$, and $x(t)$. Let $\bar{X}(t):=\E[x(t)x(t)^T]$ denote the state correlation matrix. Using the independence assumption between $x(t)$ and $\bigtriangle$, and simple algebra, \eqref{eq:var-expr} can be rewritten as 
%\begin{equation}
%\label{eq:state-correlation}
%\begin{split}
%\bar{X}(t+1) = \Azero \bar{X}(t) {\Azero}^T + \sum_{j, k \in [m]} \Sigma_{\triangle,jk} A^{(j)} \bar{X}(t) {A^{(k)}}^T + B \Sigma_{\bar{\omega}} B^T
%\end{split}
%\end{equation}
%\ksmargin{complete}
%\kscomment{For the $\Sigma_{\omega}=\zerobf$ (no additive noise), and hence $\Sigma_{\bar{\omega}}=\zerobf$ case, \cite[Chapter 9]{Boyd.ElGhaoui.ea:94} implies (a). The equivalence between (a) and (b) is known from \cite[Proposition 2.6]{Costa.Fragoso.ea:06}. (c) follows from Theorem 3.2 and Section VI in \cite{Bamieh.Filo:18}.} 
%%The equivalence between (a) and (c) follows from \cite[Theorem 6.4]{Elia:05}.
%%where we have assumed that, at a given $t$, $\gamma_i(t)$ is independent of $\{\gamma_j(t), \, j \in [n] \setminus \{i\}\}$.
%%\end{proof}

%\subsection{Proof of Proposition~\ref{prop:stable}}
%%\begin{proof}
%\ksmargin{check the proof}
%Sufficiency is easy to argue. Necessity follows from the application of Cauchy-Schwarz inequality:
%$
%|\E x_i(t) x_j(t)| \leq \sqrt{\E x_i^2(t) E x_j^2(t)}
%$.
%%\end{proof}

\subsection{Proof of Theorem~\ref{thm:unstable}}
\label{sec:unstable-proof}
%\begin{proof}
%\begin{enumerate}
%\item[(a)] 
The argument here closely follows the proof for a similar result in \cite{Wang.Elia:12}. For $\Gamma(t)=\onebf$, \eqref{eq:dynamics-original} becomes $x(t+1)=\sum_{j=0}^m \tilde{A}^{(j)} x(t) + \omega(t)$, and therefore, 
\begin{equation*}
\label{eq:Abar-def}
x(t+1)-x(t)=(\underbrace{\sum_{j=0}^m \tilde{A}^{(j)}-I}_{\Abar}) \, x(t) + \omega(t)
\end{equation*}
Without loss of generality, we provide proof only for $i=1$; the result for other states follow similarly. 
%The iteration for $x_1$ is given by:
%$$
%x_1(t+1)-x_1(t) = \bar{\Amatrix}_{1} x(t) + B_{w,1} w(t)
%$$
%where $\bar{\Amatrix}:=\Amatrix - I_n$. 
When $\Gamma(t)=\onebf$, $x_1(t+1)-x_1(t)=\Abar_1 x(t) + \omega_1(t)$ (recall that $\Abar_1$ denotes the first row of $\Abar$), which, using the independence of $x(t)$ and $\omega(t)$, implies $\left(x_1(t+1) - x_1(t) \right)^2=\Abar_{1} x(t) x^T(t) \Abar_{1}^T + \Sigma_{\omega,11} \geq \Abar_{1} x(t) x^T(t) \Abar_{1}^T=\left(\Abar_{1} x(t)\right)^2 \geq 0$. $\left(x_1(t+1) - x_1(t) \right)^2$ can be similarly shown to be non-negative for other realizations of $\Gamma(t)$. Therefore, 
$$
\E[\left(x_1(t+1) - x_1(t) \right)^2] \geq \Pr(\Gamma=\onebf) \cdot \E [\Abar_{1} x(t) x^T(t) \Abar_{1}^T ], \qquad \forall \, t \geq 0  
$$
We now show that $\lim_{t \to \infty} \E[(x_1(t)-x_1(t-1))^2] = \infty$, which then gives the theorem. Along the lines of the proof of \cite[Lemma 4]{Wang.Elia:12}, one can show that there exist $M_1 \geq 0$ and $\lambda \geq 1$ such that:
\begin{equation}
\label{eq:H-eigen-equation}
\lambda M_1 = \Azero M_1 {\Azero}^T + \sum_{j \in [m]} A^{(j)} M_1 {A^{(j)}}^T 
\end{equation}
Suppose, by contradiction, that $\Abar_{1} M_1 \Abar_{1}^T=0$. Multiplying by $\Abar_{1}$ and $\Abar^T_{1}$ on both sides of \eqref{eq:H-eigen-equation}, we get 
\begin{equation}
\label{eq:H-eigen-equation-1}
\Abar_{1} \Azero M_1 {\Azero}^T \Abar^T_{1} + \sum_{j \in [m]}  \Abar_{1} A^{(j)} M_1 {A^{(j)}}^T \Abar_{1} = \lambda \Abar_{1} M_1 \Abar^T_{1} = 0
\end{equation}
$M_1 \geq 0$ implies $\Azero M_1 {\Azero}^T \geq 0$ and $A^{(j)} M_1 {A^{(j)}}^T \geq 0$ for all $j \in [m]$. 
Therefore, \eqref{eq:H-eigen-equation-1} implies that  $\Abar_{1} \Azero M_1 {\Azero}^T \Abar^T_{1}=0$ and $\Abar_{1} A^{(j)} M_1 {A^{(j)}}^T \Abar_{1}=0$ for all $j \in [m]$. Repeatedly multiplying \eqref{eq:H-eigen-equation} by $\Azero$ on the left and by ${\Azero}^T$ on the right and then multiplying by $\Abar_{1}$ on the left and by $\Abar^T_{1}$ on the right, we get 
%$\Abar_{1} (\Azero)^p M_1 ({\Azero}^T)^p \Abar^T_{1}=0$ and $\Abar_{1} (\Azero)^p A^{(j)} M_1 {A^{(j)}}^T({\Azero}^T)^p \Abar^T_{1}=0$ for all $p \geq 0$ and $j \in [m]$. This in turn implies 
that $M_1 ({\Azero}^T)^p \Abar^T_{1}=0$ and 
\begin{equation}
\label{eq:evalue-zero}
M_1 {A^{(j)}}^T({\Azero}^T)^p \Abar^T_{1}=0, \quad \forall p \geq 0, \,  j \in [m] 
\end{equation}

%We next show that there exists at least one $j \in [m]$ such that $M_1 {A^{(j)}}^T \neq 0$. 
If there is no $j \in [m]$ such that $M_1 {A^{(j)}}^T \neq 0$, then the transfer function $C \left(zI-A \right)^{-1} B$ seen by $\bigtriangle$ is zero, and hence $CB=0$, which, from \eqref{eq:state-space-matrices}, implies the contradiction that $A^{(j)}=0$ for all $j \in [m]$. Therefore, $M_1 {A^{(j)}}^T \neq 0$ for some $j \in [m]$, and hence \eqref{eq:evalue-zero} implies:
\begin{equation}
\label{eq:postulate}
\Abar_{1} {\Azero}^p = 0, \qquad \forall \, p \geq 0
\end{equation}

We now show that \eqref{eq:postulate} can not hold true. 
If all the elements of $\Abar_{1}$ are nonzero, we get a contradiction with \eqref{eq:postulate} for $p=0$. 
Let $\Abar_{1k}=0$ for some $k \in [n]$. \eqref{eq:diag-entries} implies that $k \neq 1$. $\Abar_{1k}=0$ for $k \neq 1$ implies that there is no arc between $1$ and $k$. We next exploit the structure of $\Abar_{1} {\Azero}^p$ to show that \eqref{eq:postulate} is not true. 
%First recall that $\Amatrix=I_n + A_0 + \sum_{j \in [m]} \mu_{\gamma_j} A_j$. 
%\kscomment{
%Therefore, we have that 
%\begin{align*}
%A_{0,i} \Amatrix & = A_{0,i} + A_{0,i} A_0 + \sum_{j \in [m]} \mu_{\gamma_j} A_{0,i} A_j \\
%& = A_{0,i} + 
%\end{align*}
%}
Recall $\Abar = \sum_{j=0}^m \tilde{A}^{(j)} - I=:\tilde{A}-I$. Therefore,
\begin{equation}
\label{eq:interim-1}
\Abar_1 \Azero(k) = \left(\tilde{A}_1 - e_1^T \right)\Azero(k) = \tilde{A}_1 \Azero(k) - \Azero_{1k} = \sum_{\ell \in [n]} \tilde{A}_{1\ell} \Azero_{\ell k} - \Azero_{1k}
\end{equation}
%
%\begin{equation}
%\label{eq:A-product}
%\Abar_i \Azero = \bar{\Amatrix}_i + \bar{\Amatrix}_i \bar{\Amatrix} = \bar{\Amatrix}_i + \bar{a}_{ii} \bar{\Amatrix}_i + \sum_{j \in N_i} \bar{a}_{ij} \bar{\Amatrix}_j = \left(1+ \bar{a}_{ii}\right) \bar{\Amatrix}_i + \sum_{j \in N_i} \bar{a}_{ij} \bar{\Amatrix}_j
%\end{equation}
%where $N_i$ is the set of neighbors of $i$. 
%Note that $\bar{a}_{ij}>0$ for all $j \in N_i$, and $\bar{a}_{ii}<0$. 
The assumption that all the off-diagonal entries of $\{\tilde{A}^{(j)}\}_{j=0}^m$ have the same sign and that $\{\mu_j\}_{j \in [m]}$ are all positive implies that the signs of the off-diagonal entries of $\Azero$ and $\tilde{A}$ are the same. Therefore, $\Abar_{1k}=0$ implies $\Azero_{1k}=0$. Combining all these, we get that the second term on the right hand side of \eqref{eq:interim-1} is zero and that each entry inside the summation in the first term is non-negative. If there is an $\ell \notin \{1,k\}$ such that $\tilde{A}_{1\ell} \neq 0$ and $\Azero_{\ell k} \neq 0$ (i.e., there is a path of length 2 between $1$ and $k$), then $\Abar_1 \Azero(k)>0$ contradicting \eqref{eq:postulate}. If there is no such $\ell$, then it also implies that $\sum_{\ell \in [n]} \Azero_{1 \ell} \Azero_{\ell k}=(\Azero)^2_{1k}=0$. Therefore, 
$$
\Abar_1 (\Azero)^2(k) = \sum_{\ell \in [n]} \tilde{A}_{1 \ell} (\Azero)^2_{\ell k} - (\Azero)^2_{1k} = \sum_{\ell \in [n]} \tilde{A}_{1 \ell} (\Azero)^2_{\ell k}
$$
One can argue similarly as before that each entry in the summation has the same sign as the off-diagonal entries and that it is not zero if and only if there exists an $\ell$ such that $\tilde{A}_{1\ell} \neq 0$ and $(\Azero)^2_{\ell k} \neq 0$ (i.e., there is a path of length 3 between $i$ and $k$). If this is not the case, then one can continue with the argument until the strong connectivity assumption implies that $\bar{A}_1 (\Azero)^{\tilde{p}}(k)=0$ for some $\tilde{p}$, contradicting \eqref{eq:postulate}.


==> routing/simulations.tex <==
\section{Simulations}
Consider the setup of Example~\ref{example:linear-transportation-network}, with the $(1,1)$ entry of $A^{(0)}$ set to $-\ell_{31}$. The parameters are chosen as: $\ell_{31}=1$, $\ell_{12}=0.1$, $\ell_{32}=0$, $\ell_{23}=0.1$, $\ell_{43}=3$, $\ell_{34}=1$, $\mu_{\gamma_1}=0.1$. Figure~\ref{fig:sim} (left) is for $B_w=\zerobf$ (i.e., noiseless case), and Figure~\ref{fig:sim} (right) is for $B_{w}=0.1 \onebf$ (i.e., small additive noise). 

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.475\textwidth]{./fig/noiseless}
\includegraphics[width=0.475\textwidth]{./fig/withnoise}
\end{center}
\caption{\sf Simulation Results.}
\label{fig:sim}
\end{figure}

==> routing/stochastic-uncertainty-problem-formulation.tex <==
\section{Problem Formulation}
Consider the following linear network flow dynamics:
\begin{equation}
\label{eq:routing-discrete-time}
x(t+1) = x(t) + \tilde{A}(t)x(t) + B_w w(t)
\end{equation}
where $x \in \real_{\geq 0}^n$ is the state of the system, the routing matrix $\tilde{A}(t)$ is a matrix-valued random process, independent of $\{x(\tau), \, \tau \leq t\}$; and $w(t)$ is a scalar (for simplicity) random process, independent of $\tilde{A}(t)$. We shall consider a particular form of \eqref{eq:routing-discrete-time} using scalar-valued random processes $\gamma_1, \ldots, \gamma_m$ as follows:
\begin{align}
x(t+1) & = \left(I + A^{(0)} + A^{(1)} \gamma_1(t) + \ldots + A^{(m)} \gamma_m(t) \right) x(t) + B_w w(t) \nonumber \\
\label{eq:routing-discrete-time-reformulation}
& = \left(I + A^{(0)} + \sum_{j=1}^m \mu_{\gamma_j} A^{(j)} \right) x(t) + \left(\sum_{j=1}^m \triangle_j(t) A^{(j)} \right) x(t) + B_w w(t)
\end{align}
%where $m$ is the number of links associated with uncertainty, $\gamma_j(t):=\mu_{\gamma_j} + \triangle_j(t)$ for all $j \in [m]$, with $\mu_{\gamma_j}$ being the mean of $\gamma_j(t)$, and \kscomment{$A_0, A_1, \ldots, A_m$ are Metzler matrices.} \ksmargin{is Metzler stuff true?} \kscomment{For simplicity, we let $\gamma_j$ be Bernoulli random variables.} \ksmargin{where is this used?}

$A^{(0)}, A^{(1)}, \ldots, A^{(m)}$ can be given the following interpretation. $A^{(0)}$ corresponds to the dynamics with no uncertainty, whereas each of $A^{(j)}$, $j \in [m]$ corresponds to an uncertain link, or possibly different levels of uncertainty of the same link; see Example~\ref{example:linear-transportation-network}. Each of $A^{(0)}, A^{(1)}, \ldots, A^{(m)}$ is a Metzler matrix, and induces a sub-graph over the complete directed graph over the node set $\mc V$. We make the following standing assumption on the directed graph formed by the union of graphs induced.   

\begin{assumption}
\label{ass:connectivity}
The union of the sub-graphs induced by $A^{(0)}, A^{(1)}, \ldots, A^{(m)}$ is strongly connected.
\end{assumption}

To avoid triviality, we also make the following assumption.
\begin{assumption}
\label{ass:multiplicative-uncertainty}
For all $j \in [m]$, $A^{(j)} \neq 0$, $\mu_j>0$ and $\sigma_j>0$.
\end{assumption}

\begin{example}
\label{example:linear-transportation-network}
For concreteness, let us consider the following example, adapted from \cite[Example 1]{Rantzer:15}, of a linear transportation network defined over the graph shown in Figure~\ref{fig:transportation-network-example}. This graph is the union of sub-graphs induced by $A^{(0)}$ and $A^{(1)}$ defined as follows: 
\begin{align*}
A^{(0)} & = \begin{bmatrix}
-0.1-\ell_{31} & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
\ell_{31} & 0 &  - \ell_{43} & \ell_{34} \\
0 & 0 & \ell_{43} & -\ell_{34}
\end{bmatrix} \\
A^{(1)} & = 
\begin{bmatrix}
0 & \ell_{12} & 0 & 0 \\
0 & -\ell_{12} - \ell_{32} & \ell_{23} & 0 \\
0 & \ell_{32} & -\ell_{23} & 0 \\
0 & 0 & 0 & 0
\end{bmatrix}
\end{align*}
where $\ell_{ij} \geq 0$ for all $i, j$.

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.4\textwidth]{./fig/linear-transportation-network}
%\begin{minipage}[c]{.4\textwidth}
%\begin{center}
%\includegraphics[width=0.7\textwidth]{./fig/uncertainty-block-diagram} \\ (a)
%\end{center}
%\end{minipage}
%\hspace{0.25in}
%\begin{minipage}[c]{.4\textwidth}
%\begin{center}
%\includegraphics[width=0.9\textwidth]{./fig/MSS-feedback} \\ (b)
%\end{center}
%\end{minipage}
\end{center}
\caption{\sf A transportation network example.}
\label{fig:transportation-network-example}
\end{figure}
\end{example}

\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.4\textwidth}
\begin{center}
\includegraphics[width=0.7\textwidth]{./fig/uncertainty-block-diagram} \\ (a)
\end{center}
\end{minipage}
\hspace{0.25in}
\begin{minipage}[c]{.4\textwidth}
\begin{center}
\includegraphics[width=0.9\textwidth]{./fig/MSS-feedback} \\ (b)
\end{center}
\end{minipage}
\end{center}
\caption{\sf (a) Linear systems with both additive and multiplicative stochastic disturbances; (b) feedback interconnection used for Definition~\ref{def:MSS-feedback}.}
\label{fig:uncertainty-block-diagram}
\end{figure}

\eqref{eq:routing-discrete-time-reformulation} can be rewritten as interconnection between a structured uncertainty and a deterministic system (cf. Figure~\ref{fig:uncertainty-block-diagram}): \ksmargin{notations in Fig~\ref{fig:uncertainty-block-diagram} need to be made consistent}
\begin{equation}
\label{eq:structured-uncertainty-form}
\begin{split}
x(t+1) & = \Amatrix x(t) + B_{u} u(t) + B_w w(t) \\
y(t) & = C x(t) \\
u(t) & = \bigtriangle(t) y(t)
%u(t) & = \bar{\triangle}(t) y(t)
\end{split}
\end{equation}
Comparing \eqref{eq:routing-discrete-time-reformulation} and \eqref{eq:structured-uncertainty-form} gives:
\begin{equation}
\label{eq:state-space-matrices}
\begin{split}
\Amatrix & = I + A^{(0)} + \sum_{j=1}^m \mu_{\gamma_j} A^{(j)}, \quad B_u = [I_n \, \, I_n \, \ldots \, I_n], \quad C = [A^{(1)} \, \, A^{(2)} \, \ldots \, A^{(m)}]^T \\
\bigtriangle(t)  & = \begin{bmatrix} \triangle_1(t) \cdot I_n & & \\ & \triangle_2(t) \cdot I_n & \\ & \ldots & \\ & & \triangle_m(t) \cdot I_n \end{bmatrix}
\end{split}
\end{equation}
Corresponding to our assumption that $w(t)$ is scalar, $B_w$ is a column vector. 
%For simplicity, we assume that $w(t)$ is scalar, and accordingly $\bar{B}$ is a column vector. 

The representation~\eqref{eq:structured-uncertainty-form} can be seen as the interconnection between the structured uncertainty $\bigtriangle$ and a deterministic system $G_w$ with the following state space matrices:
\begin{equation*}
G_w: 
\left[\begin{array}{c|c|c}
\Amatrix & B_u & B_w \\
\hline
C & 0 & 0 
\end{array} \right]
\end{equation*}
We call the system seen by $\bigtriangle$ the mean system and denote it by $G$:
\begin{equation}
\label{eq:mean-system}
G: 
\left[
\begin{array}{c|c}
\Amatrix & B_u \\
\hline
C & 0
\end{array}
\right]
\end{equation}

Recall the independence assumptions on $\{\triangle_j\}_{j \in [m]}$ and $w(t)$. Accordingly, let
$$
\Sigma = \begin{bmatrix} \sigma^2_{\gamma_1} \cdot I_n & & \\ & \sigma^2_{\gamma_2} \cdot I_n & \\ & \ldots & \\ & & \sigma^2_{\gamma_m} \cdot I_n \end{bmatrix}
$$
be the covariance matrix of $\bigtriangle$. We assume that $w(t)$ has zero mean and variance $\sigma_w^2$. Our objective is to find (tight) conditions on $A^{(0)}$, $A^{(1)}, \ldots, A^{(m)}$, $\{\sigma^2_{\gamma_j}\}_{j \in [m]}$, $\Sigma$ and $\sigma_w^2$  to ensure that \eqref{eq:structured-uncertainty-form} is mean square stable. 

\begin{definition}
A causal linear time invariant system $\mathcal M$ is called \emph{Mean-Square Stable} (MSS) if for each white, second-order input process $u$ with uniformly bounded variance, the output process $y=\mathcal M u$ has uniformly bounded variance
$$
y_t := E[y_t y_t^*] \leq c \left(\sup_{\tau} \, u_{\tau} \right)
$$ 
with $c$ a constant independent of $t$ and the process $u$.
\end{definition}

\ksmargin{Definition~\ref{def:MSS-feedback} probably redundant}
The above definition is extended to feedback interconnections as follows.
\begin{definition}
\label{def:MSS-feedback}
Consider the feedback system of Figure~\ref{fig:uncertainty-block-diagram} with $d$ and $w$ being white second order processes, and $\mc M$ and $\mc G$ causal LTI systems. The feedback system in Figure~\ref{fig:uncertainty-block-diagram} is called mean-square stable if all signals $u$, $y$, $v$ and $r$ have uniformly bounded variance sequences, i.e., if there exists constant $c$ such that
$$
\max \left\{\|u\|_{\infty}, \|y\|_{\infty}, \|v\|_{\infty}, \|r\|_{\infty} \right\} \leq c \, \min \left \{\|d\|_{\infty},\|w\|_{\infty} \right \}
$$
\end{definition}




==> routing/unstable-theorem-optional.tex <==
The next result provides a characterization of unstable behavior for arbitrary $\omega(t)$, however under the special setting of network dynamics with unreliable links in Section~\ref{sec:applications}. 
%In preparation for this result, we recall the equivalence between matrix and network structure outlined in Section~\ref{sec:notations} and utilized in Section~\ref{sec:asymptotic-dynamical} implies that the stochastic uncertainty in \eqref{eq:dynamics-non-asymptotic} can be interpreted in terms of uncertainty in the network structure. 
Let $\{\mc G^{(j)} = (\mc V, \mc E^{(j)}, \mc W^{(j)})\}_{j=0}^m$ be the corresponding networks, where $\mc V$ is the superset of all the nodes,  with $|\mc V|=n$, and $\mc W^{(j)} = A^{(j)}$ for all $j=0, 1, \ldots, m$, are all $n \times n$ weight matrices. 
%The following is the natural extension of (A1) from Section~\ref{sec:notations} to the current setting:
%\begin{enumerate}
%\item[(A1-e)] The union of the graphs $\mc G^{(0)}, \mc G^{(1)}, \ldots, \mc G^{(m)}$ is strongly connected.
%\end{enumerate}

\begin{theorem}
\label{thm:unstable}
%Consider the network flow dynamics described in Section~\ref{sec:network-flow-example}. 
Consider the setting of Section~\ref{sec:applications} with uncorrelated uncertainties, i.e., diagonal $\Sigma_{\Gamma}$. Let the union of the graphs $\{\mc G^{(j)}\}_{j=0}^m$ be strongly connected, the off-diagonal entries of all $\{\tilde{A}^{(j)}\}_{j=0}^m$ be all of the same sign, 
and 
\begin{equation}
\label{eq:diag-entries}
\sum_{j=0}^m \tilde{A}^{(j)}_{ii} \neq 1, \qquad \forall \, i \in [n]
\end{equation}
%
%\begin{equation}
%\label{eq:prob-lower-bound}
%\exists \, \delta>0, \epsilon>0 \text{ s.t. }\Pr(|\triangle_j|>\delta)>\epsilon \quad \forall \, j \in [m]
%\end{equation}
If \eqref{eq:structured-uncertainty-form} is not MS stable, then $\lim_{t \to \infty} \E[(x_i(t)-x_i(t-1))^2] = \infty$ for all $i \in \mc V$.
%The following results hold true.
%\begin{enumerate} 
%\item[(a)] 
%$\lim_{t \to \infty} E[x_i(t)] = \infty$ and 
%\item[(b)] Let \kscomment{$\eta < 0$}. \kscomment{$x_i(t)$ (or $x_i(t)-x_i(t-1)$?)} converges in distribution to a random variable $R_i$, for all $i \in \mc V$, as $t \to \infty$. Furthermore, $R_i$ has unbounded second moment if and only if \eqref{eq:structured-uncertainty-form} is MS unstable.
%\end{enumerate}
\end{theorem}

The proof of Theorem~\ref{thm:unstable} is provided in Section~\ref{sec:unstable-proof}. 


%\ksmargin{simulations need revision ... because spectral radius is one; perhaps best to remove the simulations altogether}
%As an illustration, consider the setting of Figure~\ref{fig:stoch-uncertainty-illustration} with $a^{(0)}_{31}=a^{(0)}_{34}=1=1-a^{(0)}_{11}=1-a^{(0)}_{44}$, $a^{(0)}_{43}=3=1-a^{(0)}_{33}$, $a^{(1)}_{12}=a^{(1)}_{23}=0.1=1-a^{(1)}_{22}=1-a^{(1)}_{33}$, and $a^{(2)}_{32}=0=1-a^{(2)}_{33}$. These choice of parameters satisfy the constraints in Section~\ref{sec:network-flow-example}. Let $\gamma_1(t)=\gamma_2(t)$, with $\mu=[0.1 \, 0.1]^T$, and hence $\Sigma_{\Gamma}=0.09 \, \onebf_2 \onebf_2^T$. Figure~\ref{fig:sim} (left) is for $\Sigma_{\omega}=\zerobf$, and Figure~\ref{fig:sim} (right) is for $\Sigma_{\omega}=0.01 \, \onebf_4 \onebf_4^T$.
%
%\begin{figure}[htb!]
%\begin{center}
%\begin{minipage}[c]{.475\textwidth}
%\begin{center}
%\includegraphics[width=0.75\textwidth]{./fig/noiseless}
%\end{center}
%\end{minipage}
%\begin{minipage}[c]{.475\textwidth}
%\begin{center}
%\includegraphics[width=0.75\textwidth]{./fig/withnoise}
%\end{center}
%\end{minipage}
%\end{center}
%\caption{\sf An illustration of unstable behavior for the network flow dynamics described in Section~\ref{sec:network-flow-example}.}
%\label{fig:sim}
%\end{figure}
